Tonal partition algebras: fundamental and geometrical aspects of representation theory

For $l,n \in \mathbb{N}$ we define tonal partition algebra $P^l_n$ over $\mathbb{Z}[\delta]$. We construct modules $\{ \Delta_{\underline{\mu}} \}_{\underline{\mu}}$ for $P^l_n$ over $\mathbb{Z}[\delta]$, and hence over any integral domain containing $\mathbb{Z}[\delta]$ that is a $\mathbb{Z}[\delta]$-algebra (such as $\mathbb{C}[\delta]$), that pass to a complete set of irreducible modules over the field of fractions. We show that $P^l_n$ is semisimple there. That is, we construct for the tonal partition algebras a modular system in the sense of Brauer [6]. (The aim is to investigate the non-semisimple structure of the tonal partition algebras over suitable quotient fields of the natural ground ring, from a geometric perspective.) Using a `geometrical' index set for the $\Delta$-modules, we give an order with respect to which the decomposition matrix over $\mathbb{C}$ (with $\delta \in \mathbb{C}^{\times}$) is upper-unitriangular. We establish several crucial properties of the $\Delta$-modules. These include a tower property, with respect to $n$, in the sense of Green [20, \S 6] and Cox $\textit{ et al}$ [8]; contravariant forms with respect to a natural involutive antiautomorphism; a highest weight category property; and branching rules.

==> tex/ep3brex0.tex <==
% $Id: prereqisites.tex,v 1.1 $
% extract migrated to rb.tex ->  ep3.tex ->  ep3branch.tex

\newcommand{\mule}{\underline{\mu}}
\newcommand{\mula}{\mu,\lambda}
\newcommand{\mulax}{\lambda,\mu}
\newcommand{\mux}[2]{(#2,#1)}
\newcommand{\spechtx}[2]{\specht_{#2,#1}}
\newcommand{\rb}[2]{\raisebox{#1}{#2}}
\newcommand{\rest}{{\mathtt {res}}} %% restriction
\newcommand{\ind}{{\mathtt {ind}}}
\newcommand{\rad}{{\mathtt {rad}}}

\subsection{Examples: applications of modularity}
%{{{ example1

%}}}
%{{{ ind res  G lemma
 \begin{example}
  Let $k=\mathbb{C}$. %Then  $\rad(\mathcal{S}^{3}_{((1),\emptyset)})\simeq \mathcal{S}^{3}_{((1),(1))}$ as a left $P^2_3(1)$-module. Hence $\mathcal{S}^{3}_{((1),\emptyset)}$ is  not simple.  
  We have the follwoing short exact sequence  of $P^2_3(1)$-modules
%  $$0\to \mathcal{S}^{3}_{((1),\phi)}+\mathcal{S}^{3}_{((1),(1))}\to \res_3(\mathcal{S}^{4}_{((2),\phi)})\to \mathcal{S}^{3}_{((2,1),\phi)}\to0 $$
\begin{equation}\label{nsses}
0\to \specht^{3}_{((1),(0))}\to \rest_3(\specht}^{4}_{((0),(1))})\to \specht^{3}_{((1),(1))}\to0.
\end{equation}
 When $\delta=1$ by finding the  kernel of the gram matrix of $\specht^{3}_{((1),(0))}$ one can show that  $\rad(\specht^{3}_{((1),(0))})\simeq \specht^{3}_{((1),(1))}$ as 
 a left $P^2_3(1)$-module.   Hence 
  $$Hom(P^3_{((1),(1))}, \rest_3(\specht^{4}_{((0),(1))}))\neq0.$$
 The Brauer-Humphreys reciprocity implise that $$(P^3_{((1),(1))}: \specht^{3}_{((1),(0))})=[ \specht^{3}_{((1),(0))}: \specht^{3}_{((1),(1))}]\neq0$$ and $$(P^3_{((1),(1))}: \specht^{3}_{((1),(1))})\neq0.$$
  Hence  $\specht^{3}_{((1),(1))}$ and  $\specht^{3}_{((1),(0))}$ are filtration factors of $P^3_{((1),(1))}$.
The functor $\ind_n(-)$ preserves the projectivity and $\rest_3(\mathcal{S}^{4}_{((0),(1))})=\ind_2(\specht^{2}_{((0),(1))})$, this means $\rest_3(\specht^{4}_{((0),(1))})$ is projective as a left $P^2_3(1)$-module. Therefore  $P^3_{((1),(1))}$ is isomorphic to $\rest_3(\specht^{4}_{((0),(1))})$ as a left $P^2_3(1)$-module. We know $P^3_{((1),(1))}$ is indecomposable, so the sequence \ref{nsses} does not split.
  \end{example}




%{{{ Local Variables
% Local Variables:
% folded-file: t
% End:
%}}}


==> tex/figs.tex <==
% $Id: figs.tex,v 1.1 $

\section{Catalogue of available figures}

\includegraphics[width=4.2in]{latexdraw/gbofs.eps}
\includegraphics[width=2in]{latexdraw/gelem.eps}
\includegraphics[width=2in]{latexdraw/glg.eps}


%{{{ Local Variables

% Local Variables:
% folded-file: t
% End:

%}}}


==> tex/qh.chwas.tex <==

\section{Quasi-heredity of $P^l_n$}
%{{{ lem
%\begin{lemma}
{\mlem{
Let $k=\C$.
Unless $\delta =0$ and $l\mid n$ the algebra $P^l_n$ is
quasi-hereditary with the heredity chain 
\beq \label{eq:hc1}
%J_{(n,0,\cdots,0)}\supset J_{(n-l,0,\cdots,0)}\supset
%J_{(n-2l,0,\cdots,0)} \supset \cdots\supset J_{(l+b,0,\cdots,0)}\supset
%J_{(b,0,\cdots,0)} \supset 0
J_{n}\supset J_{n-l}\supset
J_{n-2l} \supset \cdots\supset J_{l+b}\supset
J_{b} \supset 0
\eq
%\red{your $n-1$ does not make sense and what is ... !!!? and what is
  %last term?? (before 0 I added to match defn!)}
%$$(a^{(n,0,\cdots,0)},a^{(n-1,0,\cdots,0)},\cdots,a^{(0,0,\cdots,0)})$$
where
%$J_\mm = P^l_n a^{\mm} P^l_n$,
$J_r = P^l_n a^{(r,0,...,0)} P^l_n$,
and 
$b$ is the remainder in $n/l$  (i.e. $n = al+b$).
\red{there are too many b's in the section}
%and the
%$h^{\text{th}}$ component of $(0,\dots0,1,0,\cdots,0)$ is the only non-zero component, 

}}
%\end{lemma}

%}}}
%{{{ proof

\red{It feels to me that the following can be expressed as a special
  case of a more general argument. Is this not true?}

\begin{proof}
% Similar ot Lemma~\ref{1.1}
We show that (\ref{eq:hc1}) is a heredity chain
in the sense of (\ref{de:qh})H1-3.
%Let $\delta\neq0$ or $l\nmid n$.
\newcommand{\ld}{l}   % convert the nonsense!
Consider the $j$th step in the chain.
Write    $r=n-jl$,   %$J_r=J_{(r,0,\cdots,0)}$    %$l\leq r\leq n$
and $P_n^{/r} = P^l_n / J_{r-\ld} $. 
We see that  $J_r/ J_{r-\ld} $
%\red{
%yours does not make sense unless $r=n-jl$ for some $j$... 
 % what is $d$ --- I assume it is $\ld$.  ??? }
is an  ideal of
$P_n^{/r} $%$P^l_n/ J_{(r-\ld,0,\cdots,0)}$ 
generated by
$a^{(r,0,\cdots,0)}+J_{r-\ld}$.
If  $\delta\neq0$ or $r \neq 0$   %$l\nmid n$
then the generator is preidempotent and we have H1.


We claim     %(similar to the Equation~\ref{eq4})
$J_r/ J_{r-\ld} $
can be decomposed into direct sum of copies of
the  left  $P_n^{/r}$-module %$P^l_n/ J_{(r-\ld,0,\cdots,0)}$-module
$P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld} $.
To this end, note the following
\red{how can we note something false!?}
isomorphism of left $P_n^{/r} $-modules
\beq
J_r/J_{r-\ld} =\bigoplus_{b^\star\in B^{(r,0,\cdots,0)}} P_n^la^{(r,0,\cdots,0)}b/J_{r-\ld}
 \simeq \bigoplus_{B^{(r,0,\cdots,0)}} P_n^la^{(r,0,\cdots,0)}/J_{r-\ld},
\eq
where ${B^{(r,0,\cdots,0)}}$ is defined in Lemma~\ref{lem:tranv1}
and $b^\star$ is defined in~\ref{de:flip}.
If  $\delta\neq0$ or $r \neq 0$ the summands are projective and we have H2.

By an argument similar to what we have in the proof of Lemma~\ref{lem:groupc} we obtain 
%Furthermore,  section \ref{ss:gammalposet} \red{???} 2.2  implies that
$$
a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld}
   \simeq \Al_r
$$
as a $\mathbb{C}$-algebra.
Hence by
Lemma \ref{lem:Stanss} 
$a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld}$
is semisimple.
Consequently $P^l_n$ is quasi-hereditary.  

\medskip

%}}}
%{{{ d=0
--- --- 

Let $n=l$ and $\delta=0$ then $P:=P^l_l a^{(0,\cdots,0,1)}$ is an
indecomposable projective $P^l_l(0)$-module with
$\rad(P)\simeq\head(P)$.  Hence $P^l_l$ is not quasi-hereditary. 
\\
Let $n=2l$, the element
$e_{2l}=\{\underline{2l}\cup(\underline{2l})'\}$ is primitive
idempotent in $ P^l_{2l}(0)$. By Lemma 4.28 the module
$\mathcal{S}^{2l}_{((0),(2))}$ is simple, and  Lemma 5.4 implies that
the modules $\mathcal{S}^{2l}_{((0),(1))}$ and
$\mathcal{S}^{2l}_{((0),(0))}$ are indecomposable with simple
head. Indeed the module $\mathcal{S}^{2l}_{((0),(0))}$ is simple, and
we have $\head(P^l_{2l}(0)
e_{2l})\simeq\head(\mathcal{S}^{2l}_{((0),(1))})\simeq
\mathcal{S}^{2l}_{((0),(0))}$ and
$\rad(\mathcal{S}^{2l}_{((0),(1))})\simeq
\mathcal{S}^{2l}_{((0),(2))}$ as  left  $
P^l_{2l}(0)$-modules. Further, a composition series of $P^l_{2l}(0)
e_{2l}$ is given by the following chain; 
$$
0\subset \mathcal{S}^{2l}_{((0),(0))}\subset
\mathcal{S}^{2l}_{((0),(0))}\oplus \mathcal{S}^{2l}_{((0),(2))}\subset
P^l_{2l}(0) e_{2l}
$$
Therefore, $ P^l_{2l}(0)$ is not quasi-hereditary.
For $n=kl$ with
$k>2$, by using the functor ${G}$ the module category of  $
P^l_{2l}(0)$  can be fully embedded into the module category of
$P^l_{kl}(0)$. Hence, $P^l_{n}(0) $ is not quasi-hereditary  for any
$n=ml$, with $m\geq1$.
\end{proof}

%}}}

{
Bibliography \red{[this is tempeorary and just to know what I have cited]}

1. Klucznik, Michael, and Steffen König.
Characteristic tilting modules over quasi-hereditary algebras. Univ., 1999. 
}

%\bibliographystyle{abbrv}
%\bibliography{ref}



==> tex/qh.chwas2.tex <==

\section{Quasi-heredity of $P^l_n$}
%{{{ lem
%\begin{lemma}
%{\mlem{
%Let $k=\C$.
%Unless $\delta =0$ and $l\mid n$ the algebra $P^l_n$ is
%quasi-hereditary with the heredity chain 
%\beq \label{eq:hc1}
%%J_{(n,0,\cdots,0)}\supset J_{(n-l,0,\cdots,0)}\supset
%%J_{(n-2l,0,\cdots,0)} \supset \cdots\supset J_{(l+b,0,\cdots,0)}\supset
%%J_{(b,0,\cdots,0)} \supset 0
%J_{n}\supset J_{n-l}\supset
%J_{n-2l} \supset \cdots\supset J_{l+b}\supset
%J_{b} \supset 0
%\eq
%%\red{your $n-1$ does not make sense and what is ... !!!? and what is
%  %last term?? (before 0 I added to match defn!)}
%%$$(a^{(n,0,\cdots,0)},a^{(n-1,0,\cdots,0)},\cdots,a^{(0,0,\cdots,0)})$$
%where
%%$J_\mm = P^l_n a^{\mm} P^l_n$,
%$J_r = P^l_n a^{(r,0,...,0)} P^l_n$,
%and 
%$b$ is the remainder in $n/l$  (i.e. $n = al+b$).
%\red{there are too many b's in the section}
%%and the
%%$h^{\text{th}}$ component of $(0,\dots0,1,0,\cdots,0)$ is the only non-zero component, 
%
%}}
%%\end{lemma}
%
%%}}}
%%{{{ proof
%
%\red{It feels to me that the following can be expressed as a special
%  case of a more general argument. Is this not true?}
%
%\begin{proof}
%% Similar ot Lemma~\ref{1.1}
%We show that (\ref{eq:hc1}) is a heredity chain
%in the sense of (\ref{de:qh})H1-3.
%%Let $\delta\neq0$ or $l\nmid n$.
%\newcommand{\ld}{l}   % convert the nonsense!
%Consider the $j$th step in the chain.
%Write    $r=n-jl$,   %$J_r=J_{(r,0,\cdots,0)}$    %$l\leq r\leq n$
%and $P_n^{/r} = P^l_n / J_{r-\ld} $. 
%We see that  $J_r/ J_{r-\ld} $
%%\red{
%%yours does not make sense unless $r=n-jl$ for some $j$... 
% % what is $d$ --- I assume it is $\ld$.  ??? }
%is an  ideal of
%$P_n^{/r} $%$P^l_n/ J_{(r-\ld,0,\cdots,0)}$ 
%generated by
%$a^{(r,0,\cdots,0)}+J_{r-\ld}$.
%If  $\delta\neq0$ or $r \neq 0$   %$l\nmid n$
%then the generator is preidempotent and we have H1.
%
%
%We claim     %(similar to the Equation~\ref{eq4})
%$J_r/ J_{r-\ld} $
%can be decomposed into direct sum of copies of
%the  left  $P_n^{/r}$-module %$P^l_n/ J_{(r-\ld,0,\cdots,0)}$-module
%$P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld} $.
%To this end, note the following
%\red{how can we note something false!?}
%isomorphism of left $P_n^{/r} $-modules
%\beq
%J_r/J_{r-\ld} =\bigoplus_{b^\star\in B^{(r,0,\cdots,0)}} P_n^la^{(r,0,\cdots,0)}b/J_{r-\ld}
% \simeq \bigoplus_{B^{(r,0,\cdots,0)}} P_n^la^{(r,0,\cdots,0)}/J_{r-\ld},
%\eq
%where ${B^{(r,0,\cdots,0)}}$ is defined in Lemma~\ref{lem:tranv1}
%and $b^\star$ is defined in~\ref{de:flip}.
%If  $\delta\neq0$ or $r \neq 0$ the summands are projective and we have H2.
%
%By an argument similar to what we have in the proof of Lemma~\ref{lem:groupc} we obtain 
%%Furthermore,  section \ref{ss:gammalposet} \red{???} 2.2  implies that
%$$
%a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld}
%   \simeq \Al_r
%$$
%as a $\mathbb{C}$-algebra.
%Hence by
%Lemma \ref{lem:Stanss} 
%$a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{r-\ld}$
%is semisimple.
%Consequently $P^l_n$ is quasi-hereditary.  
{\mlem{
Let $k=\C$. Define a partial order relation $\leq$ on $\Lambda(P^l_n)$
 by $\underline\mu\leq_\Delta\underline\nu$ implies $\underline\nu\leq\underline\mu$, where $\leq$ is defined in \ref{de:remcx}.  Unless $\delta =0$ and $l\mid n$ the algebra $(P^l_n,\leq_\Delta)$ is
quasi-hereditary with the set of standard modules 
$\{ \specht_{\lmu} \; | \; \lmu \in \Lambda(P^l_n) \}$. 
%with the heredity chain 
%\beq \label{eq:hc1}
%%J_{(n,0,\cdots,0)}\supset J_{(n-l,0,\cdots,0)}\supset
%%J_{(n-2l,0,\cdots,0)} \supset \cdots\supset J_{(l+b,0,\cdots,0)}\supset
%%J_{(b,0,\cdots,0)} \supset 0
%J_{n}\supset J_{n-l}\supset
%J_{n-2l} \supset \cdots\supset J_{l+b}\supset
%J_{b} \supset 0
%\eq
%\red{your $n-1$ does not make sense and what is ... !!!? and what is
  %last term?? (before 0 I added to match defn!)}
%$$(a^{(n,0,\cdots,0)},a^{(n-1,0,\cdots,0)},\cdots,a^{(0,0,\cdots,0)})$$
%where
%$J_\mm = P^l_n a^{\mm} P^l_n$,
%$J_r = P^l_n a^{(r,0,...,0)} P^l_n$,
%and 
%$b$ is the remainder in $n/l$  (i.e. $n = al+b$).
%\red{there are too many b's in the section}
%and the
%$h^{\text{th}}$ component of $(0,\dots0,1,0,\cdots,0)$ is the only non-zero component, 

}}
%\end{lemma}

%}}}
%{{{ proof

\red{It feels to me that the following can be expressed as a special
  case of a more general argument. Is this not true?}
\begin{proof}
We prove the result by showing that $(P^l_n,\leq_\Delta)$ with the given set of modules satisfies the conditions of the definition of the quasi-hereditary in the sense \red{{cite CPS???}}. By Theorem~\ref{de:remcx} we have the first condition of  the definition. The second condition follows from Equation~\ref{eq:BH1}.  \red{I think we need to move eq \ref{eq:BH1} to somewhere before this result}

%\medskip

%}}}
%{{{ d=0
Let $n=l$ and $\delta=0$  then $P:=P^l_l a^{(0,\cdots,0,1)}$ is an
indecomposable projective $P^l_l(0)$-module with
$\rad(P)\simeq\head(P)$.  Hence $P^l_l$ is not quasi-hereditary. 
\\
Let $n=2l$, the element
$e_{2l}=\{\underline{2l}\cup(\underline{2l})'\}$ is primitive
idempotent in $ P^l_{2l}(0)$. %By Lemma ?? the module $\mathcal{S}^{2l}_{(0,\cdots,0,(2))}$ is simple, and  
Equation~\ref{eq:spechtinflate} implies that
the modules $\mathcal{S}^{2l}_{(0,\cdots,0,(1))}$ and
$\mathcal{S}^{2l}_{(0,\cdots,0)}$ are indecomposable with simple
head. Indeed by doing some linear algebra calculations one can show that the module $\mathcal{S}^{2l}_{(0,\cdots,0)}$ is simple, and $\head(P^l_{2l}(0)
e_{2l})=\head(\mathcal{S}^{2l}_{(0,\cdots,0,(1))})\simeq
\mathcal{S}^{2l}_{(0,\cdots,0)}$. 
% and $\rad(\mathcal{S}^{2l}_{(0,\cdots,0,(1))})\simeq \mathcal{S}^{2l}_{(0,\cdots,0,(2))}$ as  left  $P^l_{2l}(0)$-modules. 
 We also have   $ \mathcal{S}^{2l}_{(0,\cdots,0)}\subset P^l_{2l}(0)
e_{2l}$, this implies $[P^l_{2l}(0)
e_{2l}:\head(P^l_{2l}(0))
e_{2l})]=2$.  
%is given by the following chain; 
%$$0\subset \mathcal{S}^{2l}_{(0,\cdots,0)}\subset
%\mathcal{S}^{2l}_{(0,\cdots,0)}\oplus \mathcal{S}^{2l}_{(0,\cdots,0,(2))}\subset
%P^l_{2l}(0) e_{2l}
%$$
Therefore, $ P^l_{2l}(0)$ is not quasi-hereditary.

For $n=kl$ with
$k>2$, by using the functor ${G}$ the module category of  $
P^l_{2l}(0)$  can be fully embedded into the module category of
$P^l_{kl}(0)$. Hence, $P^l_{n}(0) $ is not quasi-hereditary  for any
$n=ml$, with $m\geq1$.
\end{proof}

%}}}

{
Bibliography \red{[this is tempeorary and just to know what I have cited]}

1. Klucznik, Michael, and Steffen König.
Characteristic tilting modules over quasi-hereditary algebras. Univ., 1999. 
}

%\bibliographystyle{abbrv}
%\bibliography{ref}



==> tex/qh.chwas3.tex <==

\section{Total order on $\gammal$}

\includegraphics[width=1.72in]{xfig/l=3.eps}


We define another order $\rhd$ on $\gammal$ as follows; let $\mm, \mm'\in \gammal$ then $\mm'\rhd\mm$ if either \\
 (1) $\#(a^{\mm})<\#(a^{\mm'})$,  or\\
 (2)  $\#(a^{\mm})=\#(a^{\mm'})$ and $\mm'<_{lex}\mm$, where $<_{lex}$ is the lexicographical order on $\mathbb{N}^l$. %Then we have the following Lemma

{\mlem{ 
 (I)The relation $\unlhd$ is a total order relation on the set $\gammal$. 
 (II) The relation $\unlhd$ is a refinement of the order $\leq$ defined on $\gammal$ in \ref{de:gammal}. 
 }}
 
 
 
 \noindent
Proof: I) This part follows from the fact that $\#(a^{\mm})<\#(a^{\mm'})$ or  $\#(a^{\mm})=\#(a^{\mm'})$ for any $\mm', \mm\in\gammal$.
 \\ II)  Let $\mm< \mm'$. Then from the definition of $\leq$ we have $\#(a^{\mm})<\#(a^{\mm'})$.
\qed
\\
\noindent 
 For example, let $l=2$ then 
\[
 (n,0)\rhd(n-2,1)\rhd(n-4,2)\rhd(n-2,0)\rhd(n-6,3)\rhd(n-4,1)\rhd(n-8,4)\]
\[ \rhd(n-6,2)\rhd(n-4,0)\rhd\cdots\rhd(0,0)/(1,0).\]
 If $l=3$ then
 \[
 (n,0,0)\rhd(n-2,1,0)\rhd(n-4,2,0)\rhd (n-3,0,1)\rhd(n-6,3,0)\rhd(n-5,1,1)\rhd(n-3,0,0)\]
\[ \rhd(n-8,4,0)\rhd(n-7,2,1)\rhd(n-6,0,2)\rhd(n-5,1,0)\cdots \rhd(1,0,0)/(0,1,0)/(0,0,0).\]



For convenience define $\mm(1), \mm(2) , ...$ as the elements of
$\gammal$ in the total order $\unlhd$.

\mdef CLAIM: For each $1\leq i\leq |\gammal|$ we have $J_{\mm(i)}\supseteq{I^{<\mmp}}$.



\noindent
Proof:
It is enough to show that  $\mm<\mm(i+1)$ implies $\mm\unlhd \mm(i)$.
But  $\mm<\mm(i+1)$ implies $\mm\lhd \mm(i+1)$.
And
$\mm \lhd \mm(i+1)$ implies $\mm \unlhd \mm(i)$.
\qed

\red{
REDUNDANT!?:
\\
Consider the following two cases:
\\
Case I) If $\#(a^{\mm(i)})<\#(a^{\mm(i+1)})$ then
for each $\mm<\mm(i+1)$  %such that $\mm\neq\mm(i)$
we have $\mm\lhd \mm(i+1)$. %Thus  $J_{\mm(i)}\supseteq{I^{<\mmp}}$.
But
$\mm \lhd \mm(i+1)$ implies $\mm \unlhd \mm(i)$.
%there is no $\mm'$ such that $\mm(i)\lhd\mm'\lhd\mm(i+1)$,
\\
Case II) If $\#(a^{\mm(i)})=\#(a^{\mm(i+1)})$  %and $\mm(i+1)<_{lex}\mm(i)$
then for each $\mm<\mm(i+1)$ we have $\#(a^{\mm})<\#(a^{\mm(i)})$.
Hence $\mm\lhd\mm(i)$.
% and this also implies $J_{\mm(i)}\supseteq{I^{<\mmp}}$.
\qed
}



==> tex/qh.tex <==

\section{Quasi-heredity of $P^l_n$}
%{{{ lem
%\begin{lemma}
{\mlem{
Let $k=\C$. The algebra $P^l_n$ is quasi-hereditary  with the heredity chain 
$$
J_{(n,0,\cdots,0)}\supset J_{(n-l,0,\cdots,0)}\supset
J_{(n-2l,0,\cdots,0)} \supset \cdots\supset
J_{(b,0,\cdots,0)} \supset \red{???}
J_{(0,\cdots0,1,0,\cdots,0)} \supset 0
$$
\red{your $n-1$ does not make sense and what is ... !!!? and what is
  last term?? (before 0 I added to match defn!)}
%$$(a^{(n,0,\cdots,0)},a^{(n-1,0,\cdots,0)},\cdots,a^{(0,0,\cdots,0)})$$
where
$J_\mm = P^l_n a^{\mm} P^l_n$,
$b$ is the remainder in $n/l$ 
(i.e. $n = al+b$),
and the
$h^{\text{th}}$ component of $(0,\dots0,1,0,\cdots,0)$ is the only non-zero component, 
unless $\delta =0$ and $l\mid n$.
}}
%\end{lemma}

\red{It feels to me that the following can be expressed as a special
  case of a more general argument. Is this not true?}

\begin{proof}
% Similar ot Lemma~\ref{1.1}
We show that the given chain is a heredity chain
(in the sense of (\ref{de:qh})H1-3).
Let $\delta\neq0$ or $l\nmid n$.
\newcommand{\ld}{l}   % convert the nonsense!
Consider the $j$th step in the chain. Write    $r=n-jl$.    %$l\leq r\leq n$
Write $P^/ = P^l_n / J_{(r-\ld,0,\cdots,0)} $. 
We see that  $J_{(r,0,\cdots,0)}/ J_{(r-\ld,0,\cdots,0)} $
\red{
yours does not make sense unless $r=n-jl$ for some $j$... 
  what is $d$ --- I assume it is $\ld$.  ??? }
is an idempotent ideal of
$P^l_n/ J_{(r-\ld,0,\cdots,0)}$ generated by
$a^{(r,0,\cdots,0)}+J_{(r-\ld,0,\cdots,0)}$.

We claim
(similar to the Equation~\ref{eq4})
$J_{(r,0,\cdots,0)}/ J_{(r-\ld,0,\cdots,0)}$
can be decomposed into direct sum of copies of
the projective left  $P^l_n/ J_{(r-\ld,0,\cdots,0)}$-module
$P^l_na^{(r,0,\cdots,0)}/ J_{(r-\ld,0,\cdots,0)}$.

Furthermore,  section \ref{ss:gammalposet} \red{???} 2.2  implies that
$$
a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{(r-\ld,0,\cdots,0)}
   \simeq \Al_r
$$
as a $\mathbb{C}$-algebra.
Hence by
Theorem \ref{th:} 4.29
$a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)}$
is semisimple.
Consequently $P^l_n$ is quasi-hereditary.  

%}}}
%{{{ d=0
---

Let $n=l$ and $\delta=0$ then $P:=P^l_l a^{(0,\cdots,0,1)}$ is an
indecomposable projective $P^l_l(0)$-module with
$\rad(P)\simeq\head(P)$.  Hence $P^l_l$ is not quasi-hereditary. 
\\
Let $n=2l$, the element
$e_{2l}=\{\underline{2l}\cup(\underline{2l})'\}$ is primitive
idempotent in $ P^l_{2l}(0)$. By Lemma 4.28 the module
$\mathcal{S}^{2l}_{((0),(2))}$ is simple, and  Lemma 5.4 implies that
the modules $\mathcal{S}^{2l}_{((0),(1))}$ and
$\mathcal{S}^{2l}_{((0),(0))}$ are indecomposable with simple
head. Indeed the module $\mathcal{S}^{2l}_{((0),(0))}$ is simple, and
we have $\head(P^l_{2l}(0)
e_{2l})\simeq\head(\mathcal{S}^{2l}_{((0),(1))})\simeq
\mathcal{S}^{2l}_{((0),(0))}$ and
$\rad(\mathcal{S}^{2l}_{((0),(1))})\simeq
\mathcal{S}^{2l}_{((0),(2))}$ as  left  $
P^l_{2l}(0)$-modules. Further, a composition series of $P^l_{2l}(0)
e_{2l}$ is given by the following chain; 
$$
0\subset \mathcal{S}^{2l}_{((0),(0))}\subset
\mathcal{S}^{2l}_{((0),(0))}\oplus \mathcal{S}^{2l}_{((0),(2))}\subset
P^l_{2l}(0) e_{2l}
$$
Therefore, $ P^l_{2l}(0)$ is not quasi-hereditary.
For $n=kl$ with
$k>2$, by using the functor ${G}$ the module category of  $
P^l_{2l}(0)$  can be fully embedded into the module category of
$P^l_{kl}(0)$. Hence, $P^l_{n}(0) $ is not quasi-hereditary  for any
$n=ml$, with $m\geq1$.
\end{proof}

%}}}

{
Bibliography \red{[this is tempeorary and just to know what I have cited]}

1. Klucznik, Michael, and Steffen König.
Characteristic tilting modules over quasi-hereditary algebras. Univ., 1999. 
}

%\bibliographystyle{abbrv}
%\bibliography{ref}



==> tex/qh1.tex <==


\newcommand{\soc}{soc}
\newcommand{\res}{{\mathbf{res}}}

\newpage

\subsection{Quasi-heredity of $\Al_n$} \label{ss:qh1}
%{{{ qh def

First we  recall the definition of quasi-heredity from [CPS]
(or see e.g. [ref 1]).

\mdef \label{de:qh}
Let $k$ be an algebraically closed field.
Fix a finite dimensional
$k$-algebra $A$.  A two sided ideal ${J}$ in $A$ is called
\textit{hereditary} ideal  if;  
\begin{enumerate}
\item[H1.] There is an idempotent $e\in A$ with $J=AeA$.
\item[H2.] $_AJ$ is a projective module.
\item[H3.] $\End_A(Ae)\simeq eAe$ is a semisimple $k$-algebra.
\end{enumerate}
The algebra $A$ is \textit{quasi-hereditary} algebra if there
is a chain of of two sided ideals 
$$
0=:  J_{0}\subset J_{1}\subset \dots\subset J_{r-1}\subset J_r:=A
$$ 
such that $J_{i+1}/J_{i}$ is a hereditary ideal in $A/J_{i}$
for  $0\leq i\leq r-1$. The above chain is called a \textit{heredity chain}.

%}}}
%{{{ A^l_n J defs

Next we construct some suitable ideals in $\Al_n$.

\mdef
For $\textbf{m}\in \mathbb{Z}^l$  define 
$$
ht(\textbf{m})=\sum_{i=1}^l{m}_i
$$
Fix $n$. 
For  $t\leq n$, we  define the following subset of $\gamma^{l,n}$
\begin{equation}\label{eq.1}
\eta_{t}  =  \{\textbf{m}\in \gamma^{l,n}\mid r_{\textbf{m}}=n
  \mbox{ and } ht(\textbf{m})=t\}.
\end{equation}
Example.
For $l=3 $ and $n=8$ we have
\beq
\eta_{8}=\{{(8,0,0)}\}, \;\;\;\;\;\;
\eta_{7}=\{{(6,1,0)}\}, \;\;\;\;
\eta_{6}=\{{(4,2,0),(5,0,1)}\},
\eq \beq
\eta_{5}=\{{(2,3,0),(3,1,1)}\}, \;\;\;
\eta_{4}=\{{(0,4,0),(1,2,1),(2,0,2)}\}, \;\;\;
\eta_{3}=\{(0,1,2)\}    %%\;\;\;\;\;\;\;\;\;\;
\eq

\newcommand{\textbfm}[2]{\textbf{m}^{#1}_{#2} } %% 

Let $\textbfm{1}{t}, \textbfm{2}{t}, \cdots ,\textbfm{|\eta_{t}|}{t}$
denote the elements of $\eta_{t}$ ordered lexicographically
(as non-negative integral vectors, with $0<1<2<...$).
\\
In our example:
$\textbfm{1}{4}=(0,4,0), \; \textbfm{2}{4}=(1,2,1), \;\; \textbfm{3}{4} = (2,0,2)$.


\newcommand{\JJ}[2]{J^{#1}_{#2}}  %% ideal hook
\newcommand{\feta}[2]{\eta^{#1}_{#2}}  %% set hook
\newcommand{\cc}{c}   %% 

For $1\leq i\leq |\eta_{t}|$ then we define
\begin{equation}\label{eq.1}
\feta{i}{t} =
\{\textbfm{1}{t}, \textbfm{2}{t}, \cdots ,\textbfm{i}{t}\},
\;\; \mbox{ and } \;\;
\cc_{i,t} = |\feta{i}{t}|  = i   .
\end{equation}
Define also the ideals in $\Al_n$
\begin{equation}\label{eq.1}
  \JJ{i}{t}
  = \sum_{\textbf{m}\in{\feta{i}{t}}} \Al_n a^{\textbf{m}} \Al_n
  \hspace{1cm}\mbox{ and }\hspace{1cm}
   \JJ{-}{t}
  = \sum_{\textbf{m}\in{\feta{}{t}}} \Al_n a^{\textbf{m}} \Al_n  .
\end{equation}
%
In our example:
$\JJ{1}{8}=\Al_8$, $\;\;$ 
$\JJ{1}{7}=\Al_8 a^{(6,1,0)} \Al_8 $, $\;\;$ 
$\JJ{2}{6}= \Al_8 a^{(4,2,0)} \Al_8 +\Al_8 a^{(5,0,1)} \Al_8$,  $\;$ 
$\JJ{1}{6} = \Al_8 a^{(4,2,0)} \Al_8,$ $\;\; \cdots, \;\;
 \JJ{1}{3} = \Al_8 a^{(0,1,2)} \Al_8$.

%}}}
%{{{ qh lem

%\begin{lemma}
{\mlem{  \label{1.1}[lemma 4.25 = \ref{th:qh1}]
Let $k=\mathbb{C}$. Then $\Al_n$ is quasi-hereditary with a heredity
chain $H$ given by 
%{{{ ignore old long-form chain
\ignore{{
\beq \nonumber
\JJ{1}{{n}}
\supset \JJ{1}{{n-1}}
\supset \JJ{{c_{|\eta_{n-2}|,n-2}}}{{n-2}} \supset 
\hspace{4in} \eq
\[ \hspace{.3in}  %\supset
\JJ{{c_{|\eta_{n-2}|-1,n-2}}}{{n-2}} + \JJ{{c_{|\eta_{n-3}|,n-3}}}{{n-3}}
%\hspace{.95in} \] \beq \nonumber
\supset \JJ{{c_{|\eta_{n-2}|-2,n-2}}}{{n-2}} + \JJ{{c_{|\eta_{n-3}|,n-3}}}{{n-3}}
\supset\dots
\supset \JJ{{{1}}}{{n-2}} + \JJ{{c_{|\eta_{n-3}|,n-3}}}{{n-3}} \;\;\;\;\;\;
\]
\beq \nonumber
\supset \JJ{{c_{|\eta_{n-3}|,n-3}}}{{n-3}}
\eq
\[
\supset \JJ{{c_{|\eta_{n-3}|-1,n-3}}}{{n-3}} + ???????
\] \[
\supset \JJ{{c_{|\eta_{n-4}|,n-4}}}{{n-4}}
\supset\dots\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;
\]
\beq
\supset \JJ{{c_{{|\eta_{h}|,h_n}}}{h_n}}
\supset \cdots\supset \JJ{1}{{h_n}} \supset 0 .
\eq
}}
%}}}
%{{{ chain
\beq \nonumber
\JJ{1}{{n}}
\supset \JJ{1}{{n-1}}
\supset \JJ{{c_{|\eta_{n-2}|,n-2}}}{{n-2}} \supset 
\hspace{4in} \eq
\[ \hspace{1.3in}  %\supset
\JJ{{c_{|\eta_{n-2}|-1,n-2}}}{{n-2}} + \JJ{-}{{n-3}}
%\hspace{.95in} \] \beq \nonumber
\supset \JJ{{c_{|\eta_{n-2}|-2,n-2}}}{{n-2}} + \JJ{-}{{n-3}}
\supset\dots
\supset \JJ{{{1}}}{{n-2}} + \JJ{-}{{n-3}} \;\;\;\;\;\;
\] \[
\supset \JJ{{c_{|\eta_{n-3}|,n-3}}}{{n-3}}
%\] \[
\supset \JJ{{c_{|\eta_{n-3}|-1,n-3}}}{{n-3}} + \JJ{-}{{n-4}} 
\supset \JJ{{c_{|\eta_{n-3}|-2,n-3}}}{{n-3}} + \JJ{-}{{n-4}} \supset
%\hspace{.1in}
\cdots %\hspace{.1in}
\supset \JJ{1}{n-3} + \JJ{-}{{n-4}}  
%\hspace{1.65in}
\] \[
\supset \JJ{{c_{|\eta_{n-4}|,n-4}}}{{n-4}}
\supset\dots \hspace{4.43in}
\]
\beq \label{eq:Hl}
\supset \JJ{{c_{{|\eta_{h_n}|,h_n}}}}{{h_n}}
\supset \cdots\supset \JJ{1}{{h_n}} \supset 0 .
\eq
%}}}
%{{{ %%%
%\begin{multline*}
%H=(a^{(n,0,\cdots,0)},a^{(n-2,1,0\dots,0)},\sum_{\textbf{m}\in\eta^{|\eta_{n,n-2}|}_{n,n-2}}a^{\textbf{m}},\sum_{\textbf{m}\in\eta^{|\eta_{n,n-2}|-1}_{n,n-2}}a^{\textbf{m}},\cdots,\sum_{\textbf{m}\in\eta^{1}_{n,n-2}}a^{\textbf{m}},\\ \sum_{\textbf{m}\in\eta^{|\eta_{n,n-3}|}_{n,n-3}}a^{\textbf{m}},\cdots,  \sum_{\textbf{m}\in\eta^{|\eta_{n,h}|}_{n,h}}a^{\textbf{m}},\cdots, \sum_{\textbf{m}\in\eta^{1}_{n,h}}a^{\textbf{m}}) \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;
%\end{multline*}
%}}}
where
\[
h_n =
\begin{cases}
n/l & \textup{if } n/l\in\mathbb{Z}
\\
\lfloor n/l\rfloor+1 & \textup{otherwise}
\end{cases}
\]
% if and only if $\delta\neq0$ or $l\nmid n$.
}}
%\end{lemma}

%}}}
%{{{ proof

\begin{proof}
We prove the lemma by showing that the given chain is a heredity chain.
%%To this end, let $h_n$ be as given in the statement of the Lemma and
Consider $h_n< k\leq n$.
From the definition of $(\gamma^{l,n},\leq)$
and (\ref{de:PPI}), 
for $1< d\leq |\eta_{n,k}|$ we have 
$$
%\left( \JJ{d}{k} + \JJ{{c_{|\eta_{k-1}|,k-1}}}{{k-1}} \right  /
% \left( \JJ{d-1}{k} + \JJ{{c_{|\eta_{k-1}|,k-1}}}{{k-1}} \right)
\left( \JJ{d}{k} + \JJ{-}{{k-1}} \right)  /
 \left( \JJ{d-1}{k} + \JJ{-}{{k-1}} \right)
 \; =\;
 P^{\textbfm{d}{k}}_n  a^{\textbfm{d}{k}} P^{\textbfm{d}{k}}_n  .
$$
 %A_n\sum_{\textbf{m}\in\eta^{d}_{n,k}}a^{\textbf{m}} A_n /
 %A_n\sum_{\textbf{m}\in\eta^{d-1}_{n,k}}a^{\textbf{m}} A_n=P^{\textbf{m}_d}_n$$
And 
$$
%\left( \JJ{1}{k} + \JJ{{c_{|\eta_{k-1}|,k-1}}}{{k-1}} \right) /
% \JJ{{c_{|\eta_{k-1}|,k-1}}}{{k-1}}
\left( \JJ{1}{k} + \JJ{-}{{k-1}} \right) /
 \JJ{-}{{k-1}}
 \; =\;  P^{\textbfm{1}{k}}_na^{{\textbfm{1}{k}}}P^{\textbfm{1}{k}}_n.
 $$
 Note that these `fully propagating' $a^\mm$s are idempotent. 
Thus the (H1) condition is satisfied.  
%$$A_n\sum_{\textbf{m}\in\eta^{1}_{n,k}}a^{\textbf{m}} A_n /
%A_n\sum_{\textbf{m}\in\eta^{|\eta_{n,k-1}|}_{n,k-1}}a^{\textbf{m}}
%A_n=P^{\textbf{m}_1}_n.$$

For any $\textbf{m}\in\gamma^{l,n}$ with $ht(\textbf{m})<h$
we have  $r_{\textbf{m}}<n$.
Hence ${\textbf{m}}\leq (n-l,0,\cdots,0)$
and $a^{\textbf{m}}=0$ in $\Al_n$.
Therefore, %$A_na^{\textbf{m}}A_n=P_n^{\textbf{m}}$
$\JJ{i}{h_n} = P_n^{\textbf{m}}a^{\textbf{m}}P_n^{\textbf{m}}$,
for any $\textbf{m}\in\eta_{h}$ and any $1\leq i\leq |\eta_{h}|$.
\\
For any $\textbf{m}\not\leq (n-l,0,0\dots,0)$ we have 
\begin{equation}\label{eq4}
  P_n^{\textbf{m}}a^{\textbf{m}}P_n^{\textbf{m}}
  \simeq \bigoplus_{b\in B_{\textbf{m}}} P_n^{\textbf{m}}a^{\textbf{m}}b
  \simeq \bigoplus_{B_{\textbf{m}}} P_n^{\textbf{m}}a^{\textbf{m}}
\end{equation}
as a left $\Al_n$-module, where
$B_{\textbf{m}}=
 \{ b \in \mP_n^{\textbf{m}} \mid a^{\textbf{m}}b\neq0_{P_n^{\textbf{m}}}\}$
 and
 $\mP_n^{\textbf{m}}$
 is defined in 2.3=\ref{de:Pnm}.
Hence the successive quotients in the given chain are projective.
The third requirement follows from Lemma 2.13=\ref{lem:213}.
\end{proof}

%}}}
%{{{ lem

%\begin{lemma}
Lem. (Lemma 2.28=\ref{lem:Stanss} of P.M doc) see the next proposition
%\end{lemma}

%\begin{proposition}
{\mpr{
  \label{stand-simp}
Let $(A,\leq)$ be a quasi-hereditary algebra with the set of standard
modules
$\{\Delta(\lambda)\mid\lambda\in \Lambda(A)\}$.
Let $\circ$ be a contavariant duality on $A$.
If each standard module is isomorphic to its contavariant dual as an
$A$-module then each standard module is simple. 
}}
%\end{proposition}

\begin{proof}
%Let each standard module $_{{T}^d_n({\delta})}\Delta_{n}(\lambda)$  be isomorphic to its contravariant dual.
Let $\lambda\in\Lambda$, in general we have 
$_{A}(\soc((\Delta(\lambda)))^\circ
\simeq {_{A}\left((\Delta(\lambda))^\circ/\rad((\Delta(\lambda))^\circ)\right)}$.
 Hence the socle of $_{A}\Delta(\lambda)$ is isomorphic to the dual of
 its $\head$.
 We claim  $_A\head(\Delta(\lambda))\simeq {_A}(\head(\Delta(\lambda)))^o$,
 hence $\head(\Delta(\lambda))\simeq \soc(\Delta_{n}(\lambda))$
 and consequently $\Delta(\lambda)$ is simple. To this end, from the   quasi-heredity of  $A$ we have $(\head(\Delta(\lambda)))^o= \head(\Delta(\lambda^\prime))$ for an  other standard module $\Delta(\lambda^\prime)$. Thus ${_A\head(\Delta(\lambda))}\simeq{_A \soc(\Delta(\lambda^\prime))}$, but by the the unitriangular property of quasi-hereditary algebras this impossible unless ${_A\Delta(\lambda^\prime)}\simeq{_A\Delta(\lambda)}$.
\end{proof}

%}}}

\newpage 


==> tex/qh2.tex <==

\section{Quasi-heredity of $P^l_n$}
%{{{ lem
%\begin{lemma}
{\mlem{
The algebra $P^l_n$ is quasi-hereditary  with the heredity chain 
$$
J_{(n,0,\cdots,0)}\supset J_{(n-1,0,\cdots,0)}\supset \cdots\supset
J_{(0,\cdots0,1,0,\cdots,0)}
$$
%$$(a^{(n,0,\cdots,0)},a^{(n-1,0,\cdots,0)},\cdots,a^{(0,0,\cdots,0)})$$
unless $\delta =0$ and $l\mid n$, where  $J_{\textup{\textbf{m}}}$ is
the ideal generated by $a^{\textup{\textbf{m}}}$ and the
$h^{\text{th}}$commponet of $(0,\dots0,1,0,\cdots,0)$ is the only the
only non-zero commponent. 
}}
%\end{lemma}
\begin{proof}
Similar ot Lemma~\ref{1.1} we show that the given chain is a heredity chain.  Let $\delta\neq0$ or $l\nmid n$. We have   $J_{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)}$ is an idempotent ideal of $P^l_n/ J_{(r-d,0,\cdots,0)}$ generated by $a^{(r,0,\cdots,0)}+J_{(r-d,0,\cdots,0)}$, where $0\leq r-l\leq r\leq n$. Simlar to the Equation~\ref{eq4}, $J_{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)}$ can be decomposed into direct sum of copies of the projective left  $P^l_n/ J_{(r-d,0,\cdots,0)}$-module $P^l_na^{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)}$. Furthermore,  section 2.2  implies that $a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)} \simeq A_r$ as a $\mathbb{C}$-algebra. Hence by Theorem 4.29 $a^{(r,0,\cdots,0)}P^l_na^{(r,0,\cdots,0)}/ J_{(r-d,0,\cdots,0)}$ is semisimple. Consequently $P^l_n$ is quasi-hereditary. 
\\Let $n=l$ and $\delta=0$ then $P:=P^l_l a^{(0,\cdots,0,1)}$ is an indecomposable projective $P^l_l(0)$-module with $\rad(P)\simeq\head(P)$.  Hence $P^l_l$ is not quasi-hereditary.
\\ Let $n=2l$, the element $e_{2l}=\{\underline{2l}\cup(\underline{2l})'\}$ is primitive idempotent in $ P^l_{2l}(0)$. By Lemma 4.28 the module $\mathcal{S}^{2l}_{((0),(2))}$ is simple, and  Lemma 5.4 implies that the modules $\mathcal{S}^{2l}_{((0),(1))}$ and $\mathcal{S}^{2l}_{((0),(0))}$ are indecomposable with simple head. Indeed the module $\mathcal{S}^{2l}_{((0),(0))}$ is simple, and  we have $\head(P^l_{2l}(0) e_{2l})\simeq\head(\mathcal{S}^{2l}_{((0),(1))})\simeq \mathcal{S}^{2l}_{((0),(0))}$ and $\rad(\mathcal{S}^{2l}_{((0),(1))})\simeq \mathcal{S}^{2l}_{((0),(2))}$ as  left  $ P^l_{2l}(0)$-modules. Further, a composition series of $P^l_{2l}(0) e_{2l}$ is given by the following chain;
$$0\subset \mathcal{S}^{2l}_{((0),(0))}\subset \mathcal{S}^{2l}_{((0),(0))}\oplus \mathcal{S}^{2l}_{((0),(2))}\subset P^l_{2l}(0) e_{2l}$$
Therefore, $ P^l_{2l}(0)$ is not quasi-hereditary.  For $n=kl$ with
$k>2$, by using the functor ${G}$ the module category of  $
P^l_{2l}(0)$  can be fully embedded into the module category of
$P^l_{kl}(0)$. Hence, $P^l_{n}(0) $ is not quasi-hereditary  for any
$n=ml$, with $m\geq1$.
\end{proof}

%}}}

\section{Restrict}
%{{{ addo remo

\newcommand{\addo}{add}
\newcommand{\remo}{rem}

Let
$
\underline\lambda=
(\lambda^1,\lambda^2,\cdots,\lambda^l)\vdash\textup{\textbf{m}}\in\gamma^{l,n+1}
$
be a multi-partition.
For $1\leq j\leq l$ we define
$\addo_j(\underline{\lambda})$ to be the set of all multi-partitions
obtained from $\underline{\lambda}$ by adding an addable box to the
Young diagram of $\lambda^{j}$, and
$\remo_j(\underline{\lambda})$ to
be the set of all multi-partitions obtained from
$\underline{\lambda}$ by removing  a removable box from the Young
diagram of $\lambda^{j}$. 

%}}}
%{{{ theorem  
 
% 
% Let $\underline\lambda=(\lambda^1,\lambda^2,\dots,\lambda^l)\vdash\textup{\textbf{m}}\in\gamma^{l,n+1}$ be a multi-partition. We define  $\textup{q}_{l-1}(\underline{\lambda})$ to be the set of all multi-partitions obtained from $\underline{\lambda}$ by adding an addable box to the Young diagram of $\lambda^{l-1}$,
%$\textup{d}_1(\underline{\lambda})$ to be  the set of all multi-partitions obtained from $\underline{\lambda}$ by removing a removable box from the Young diagram of  $\lambda^1$,
%$\textup{q}_l(\underline{\lambda})$ to be  the set of all multi-partitions obtained from $\underline{\lambda}$ by removing a removable box from the Young diagram of  $\lambda^{1}$ and adding an addable box to the Young diagram of  $\lambda^{l}$,
%and
%$\textup{s}(\underline{\lambda})$ to be the set of all multi-partitions obtained from $\underline{\lambda}$ by removing a removable box from the Young diagram of  $\lambda^{i+1}$ and adding an addable box to the Young diagram of  $\lambda^{i}$, for $1\leq i\leq l-1$. 
%%
%  \substack{\text{Some long text that} \\ \text{should be multiline}}

%\begin{theorem}
{\mth{
Let $\res_n:P^l_{n+1}-mod\to P^l_n-mod$ denote the natural
restriction corresponding to the inclusion
$P^l_n \hookrightarrow P^l_{n+1}$ given by
$d\mapsto 1\otimes d$. For
$
\underline\lambda=(\lambda^1,\lambda^2,\cdots,\lambda^l)
   \vdash\textup{\textbf{m}}\in\gamma^{l,n+1}
$
the module $\res_n(\mathcal{S}^{n+1}_{\underline\lambda})$
has a filtration by Specht modules. The multiplicities are given by  
\begin{equation*}
\res_n(\mathcal{S}^{n+1}_{\underline\lambda})
={+}_{\substack{{\underline\mu\in \addo_{i}(\remo_{i+1}(\underline\lambda))}\\ {1\leq i\leq l-1}}}                         \mathcal{S}^{n}_{\underline\mu}
+_{{\underline\mu}\in \addo_{l-1}(\underline\lambda)}
\mathcal{S}^{n}_{\underline\mu}
+_{{\underline\mu}\in \addo_l(\remo_1(\underline\lambda))}\mathcal{S}^{n}_{\underline\mu}
+_{{\underline\mu}\in \remo_1(\underline\lambda)}\mathcal{S}^{n}_{\underline\mu}
\end{equation*}
}}
%\end{theorem}

\begin{proof}
We may organise the set
$B^{\underline{\lambda}}_{\textup{sp}}$ of basis diagrams of
$\mathcal{S}^{n+1}_{\underline\lambda}$  into $l+2$ types in the
following way.
These are the subsets
$B^{\underline{\lambda}}_{\textup{sp}}(i)$,
$B^{\underline{\lambda}}_{\textup{sp}}(j^\prime)$
where $i=1,2,\cdots,l$ and $j=l,l-1$ containing diagrams in which the first vertex is:
\begin{enumerate}
\item
a ``propagating singleton'', this subset is denoted by $B^{\underline{\lambda}}_{\textup{sp}}(1)$.
%\item $B^{\underline{\lambda}}_{\textup{sp}}(1)$ contains all the diagrams where `the first vertex is a ``propagating singleton''.
%\item For $i=2,3,\cdots,l$ we let  $B^{\underline{\lambda}}_{\textup{sp}}(i)$ be the set containing all diagrams in which the first vertex is in a ``propagating part'' such that the number of vertices in the northern part  
\item part of a propagating part  $\textbf{p}$ such that $|\textbf{p}\cap \underline{n}|=i \pmod l$, this subset is denoted by $B^{\underline{\lambda}}_{\textup{sp}}(i)$ for $i=2,\cdots,l$.
\item part of a propagating part  $\textbf{p}$ such that $|\textbf{p}\cap \underline{n}|>l$ and $|\textbf{p}\cap \underline{n}|=1 \pmod l$, this subset is denoted by $B^{\underline{\lambda}}_{\textup{sp}}(l^\prime)$.
\item
  part of a non-propagating part, this subset is denoted by
  $B^{\underline{\lambda}}_{\textup{sp}}((l-1)^\prime)$.
\end{enumerate}
  
Case 1. 
  
  
%\begin{example}
\mex
\textup{Let $k=\mathbb{C}$. Then $P^2_4(1)$ and $P^2_3(1)$ are not
  semisimple, and  have the follwoing short exact sequence  of
  $P^2_3(1)$-modules 
$$
0 \to \mathcal{S}^{3}_{(\phi,(1))}\to
    \res_3(\mathcal{S}^{4}_{(\phi,(2))})\to
    \mathcal{S}^{3}_{((1),(1))}\oplus\mathcal{S}^{3}_{(\phi,(3))}
    \oplus\mathcal{S}^{3}_{(\phi,(1))}
    \to 0
$$
which is non-splite since $\res_3(\mathcal{S}^{4}_{(\phi,(2))})$ has
no proper submodule containg
$
\mathcal{S}^{3}_{((1),(1))}\oplus\mathcal{S}^{3}_{(\phi,(3))}\oplus\mathcal{S}^{3}_{(\phi,(1))}
.
$
}
%\end{example}
\end{proof}

%}}}

Bibliography [this is tempeorary and just to know what I have cited]

1. Klucznik, Michael, and Steffen König.
Characteristic tilting modules over quasi-hereditary algebras. Univ., 1999. 


%\bibliographystyle{abbrv}
%\bibliography{ref}



==> tex/qh99.tex <==
% $Id: qh99.tex,v 1.1 $


{\mlem{ \label{lem:Pfiltered}
For $\delta\neq0$, the indecomposable projective  $P^l_n $-modules are  filtered by $\Delta$-modules. 
}}

\proof \redxx{Using Lemma~\ref{lem:gentry}.}
Consider the ideal chain from \ref{id-chain}.
The sections are as in Lemma~\ref{lem:step2}.
By % Lemma~\ref{}
Equations~\ref{eq:PaP1} and ~\ref{eq:PaP2}
these are sums of certain modules, and by \ref{le:Diso} these
modules are $\Delta$-modules.
Now use Lemma~\ref{lem:gentry}.
\qed


\ignore{{

\proof
\red{Draft direct proof:}
Let $P$ be an indecomposable projective left $P^l_n$-module. Then there exist a primitive idempotent  $f\in P^n_l$ such that $P=P^l_nf$. We obtain the following chain of submodules of $P$ from~\ref{id-chain}
\begin{equation}\label{Pf-Cha}
J_{\mm(1)}f \subseteq J_{\mm(2)}f \subseteq J_{\mm(3)}f \subseteq ...\subseteq P^l_nf=P.
\end{equation}
For   $0<i\leq|\gammal|$,  % if  $J_{\mm(i-1)}f\neq J_{\mm(i)}f$ %(otherwise the factor $J_{\mm(i)}f/J_{\mm(i-1)}f$ is trivial) 
%then $J_{\mm(i)}f/J_{\mm(i-1)}f$ is non-trivial. 
the factor $J_{\mm(i)}/J_{\mm(i-1)}$ is a $P^l_n$-bimodule.


% Hence from the definition of quotient modules we obtain $J_{\mm(i)}f/J_{\mm(i-1)}f= \left(J_{\mm(i)}/J_{\mm(i-1)}\right)f.$   
We have  following short exact sequence of  $P^l_n$-bimodules
 \begin{equation}\label{ses-J_i}
0\to J_{\mm(i-1)}\xrightarrow{\iota} J_{\mm(i)}\xrightarrow{\pi } J_{\mm(i)}/J_{\mm(i-1)}\to 0.
\end{equation}
where $\iota$ is the inclusion map and $\pi$ is the "natural" surjection.   


Then the exactness of the functor $L_\eW$  and Equation~\ref{ses-J_i} implies that the following sequence is a short exact sequence of  right $fP^n_lf$-modules
\begin{equation}
0\to J_{\mm(i-1)}f\xrightarrow{\iota }  J_{\mm(i)}f\xrightarrow{\pi }  \left(J_{\mm(i)}/J_{\mm(i-1)}\right)f\to 0.
\end{equation}
Hence ???$ \left(J_{\mm(i)}/J_{\mm(i-1)}\right)f=J_{\mm(i)}f/\iota(J_{\mm(i-1)}f)=J_{\mm(i)}f/J_{\mm(i-1)}f$ %as a left $P^l_n$-module. 


Then by Lemma~\ref{lem:Mfissummand} $J_{\mm(i)}f/J_{\mm(i-1)}f$ is isomorphic to a submodule of
$J_{\mm(i)}/J_{\mm(i-1)}.$  


Further Lemma~\ref{lem:step2}, and Equations~\ref{eq:PaP1} and ~\ref{eq:PaP2} imply the following isomorphisms of left $P^l_n$-modules  
\begin{equation}J_{\mm(i)}/J_{\mm(i-1)}\cong P^{\mm(i)}_na^{\mm(i)}P^{\mm(i)}_n\cong \bigoplus_{T^{\mm(i)}}P^{\mm(i)}_na^{\mm(i) }\cong\bigoplus_{T^{\mm(i)}}\bigoplus_{\underline\mu\in\Lambda_{\mm(i) }}P^{\mm(i) }_na^{\mm(i) } e_{\underline\mu}.\end{equation}


By Krull-Schmidt theorem for modules the indecomposable direct summands of the left $P^l_n$-module $J_{\mm(i)}f/J_{\mm(i-1)}f$ are isomorphic to some of the indecomposable  direct summands of  $J_{\mm(i)}/J_{\mm(i-1)}$.   


By Lemma~\ref{le:Diso} $J_{\mm(i)}/J_{\mm(i-1)}$ is isomorphic to direct sums of
$\Delta$-modules. Thus $P$ is filtered by $\Delta$-modules.

}}


%{{{ Local Variables

% Local Variables:
% folded-file: t
% End:

%}}}


==> tex/sandpit.tex <==
% $Id: sandpit.tex,v 1.1 $

%\subsection{Chwas's sandpit}
%{{{ Chwas
\blu{%This is a description of the above \\
%Part c) for  $p\in I^{<\mm}$ we claim $p(t\otimes ww^*)\ox a\omega=0$.
\\ Proof of Claim:
(a) and (b) are routine --- see e.g. Fig.\ref{fig:1x}.
Hereafter we focus on (c).
The ideal $ I^{<\mm}$ is spanned by  partitions of the form $sa_n^{\mm'}q$ with $s,q\in \mP^l_{\underline{n}\sqcup\underline{n}}$ and $\mm'<\mm$. Hence by the definition of balanced maps it is enough to prove (c) for  $p=sa_n^{\mm'}q$ where  $\mm'<\mm $.\ignore{Then by  [  Corollary 26 in \cite{AMM1}, the Coro states: Given any partition $p\in \mP^l_{\underline{n}\sqcup\underline{n}}$ there exists $q,s, q',s'\in \mP^l_{\underline{n}\sqcup\underline{n}}$ and a unique $\mm$ such that $p=sa^{\mm}q$ and $a^{\mm}=s'pq'$] there exist $\mm'<\mm $  and $q\in P^l_{n-l}$ such that $ p(t\otimes ww^*)=sa^{\mm'}_n(q\otimes1_l )$ for some $s\in P^l_n$.}
Then 
\begin{equation} \begin{split}
p(t\otimes ww^*) &= sa_n^{\mm'}q (t\otimes ww^*)=s(a_{n-l}^{\mm'}\otimes ww^*)q (t\otimes ww^*)\\
&=s\left(\left(\left(a^{\mm'}_{n-l}\otimes w^*\right)q\left(t\otimes w\right)\right) \otimes ww^*\right).
\end{split}
\end{equation}
(NB.  by (\ref{eq:amm}) we have $a^{\mm'}_{n-l}\otimes ww^*=a^{\mm'}_{n}$). Then $\left(a^{\mm'}_{n-l}\otimes w^*\right)q\left(t\otimes w\right)=a^{\mm'}_{n-l}q'$ for some $q'\in P^l_{n-l}$, hence $p(t\otimes ww^*)=s(a^{\mm'}_{n-l}q' \otimes ww^*)$.
\ignore{, and $a^{\mm'}_{n-l}qt$ should be understood as $(a^{\mm'}_{n-l}\otimes w^*)q(t\otimes w)$}
The map defined in Theorem~\ref{th:UEU} removes the right most $ww^*$, and hence  sends  $( a^{\mm'}_{n-l}q') \otimes ww^*$ to $a^{\mm'}_{n-l}q'$. Now we can move  $( a^{\mm'}_{n-l}q') \otimes ww^*$ to the right as follows
\begin{equation}\label{eq:pww}
p(t\otimes ww^*)\ox a\omega=s(( a^{\mm'}_{n-l}q') \otimes ww^*)\ox a\omega=s\ox a^{\mm'}_{n-l}q'a\omega
\end{equation}
% ignore the following for a moment (we not need it at all)
\ignore{\begin{equation}
=\sum_{\kappa \in b_{\lmu} }\alpha_\kappa(sa_{n}^{\mm'}\ox \kappa)
=\sum_{\kappa \in b_{\lmu} } \alpha_\kappa (s\ox  a_{n-l}^{\mm'}\kappa)
\end{equation} where $\alpha_\kappa\in K$.}%end ignore
%
But the module $\specht^{n-l}_{\lmu}$ is annihilated
by
any $a^{\mm'}$ with $\mm'<\mm$. Hence  eq \ref{eq:pww} is zero.}
\red{END OF PROOF OF CLAIM.}

%}}}
\ignore{{
%{{{ dimension bit

\medskip


\mdef
\blu{May be we can use the following argument to show that
\\
CLAIM. $dim(\specht^n_{\lmu} )= dim(G_\W \; \specht^{n-l}_{\lmu})$
\\ By a, b and c the equation ?? (19) becomes 
\[= \kk \{   % ((t+ I^{<\mm}_{n-l})
         t 
            \ox a^\mm_{n-l} \www\omega 
              \; |\; t \in \pT^\mm_{n};  \omega \in b_{\lmu}  \}
\]
Hence $dim(G_\W \; \specht^{n-l}_{\lmu})\leq |\pT^\mm_{n}\times b_{\lmu}  |=dim(\specht^n_{\lmu} )$. 
\\
Claim: For any $t\in \pT^\mm$ and $ \omega \in b_{\lmu}$ we  have
$  t \ox a^\mm_{n-l} \www\omega\neq0 $.
\\
Proof: We start by showing  $  a^\mm_{n} \ox
a^\mm_{n-l} \www\omega\neq0 $ for any $ \omega \in b_{\lmu}.$ If  $
a^\mm_{n} \ox a^\mm_{n-l} \www\omega=0$ some $\omega\in b_{\lmu},$
then given any other $\tau\in b_{\lmu} $ there exist $\sigma\in \kk
S_\mm$ such that $\tau =\sigma\omega$. By (a) we have $$a^\mm_{n} \ox
a^\mm_{n-l} \www\tau=q (a^\mm_{n} \ox a^\mm_{n-l} \www\omega)=0$$
where $q$ is  the image $\sigma$ after moving it to left.  Hence
$a^\mm_{n} \ox \specht^{n-l}_{\lmu} =0$. Therefore
$P^l_n \W \ox \specht^{n-l}_{\lmu} =(P^l_n \W a^\mm_n)\ox a^\mm_{n-l}
w^{ba}_{e_\mu}=P^l_n \W (a^\mm_n\ox a^\mm_{n-l} w^{ba}_{e_\mu})=0,$ a
contradiction. Now let $t\in\pT^\mm$ then there exist  $p\in P^l_n$
(?? I have a  proof of this point is it is not clear) such that
$a^\mm_n=pt$.
Hence by the above argument  $  t \ox a^\mm_{n-l} \www\omega\neq0 $  for any   $ \omega \in b_{\lmu}.$ 
\\ (( I hope we can show that  if $t\neq t'$ then
$  t \ox a^\mm_{n-l} \www\omega \neq  t' \ox a^\mm_{n-l} \www\omega$, since if
this is true the next map would be welldefined  ))
\\ The map
\begin{equation} \begin{split}
 \{   % ((t+ I^{<\mm}_{n-l})
         t 
            \ox a^\mm_{n-l} \www\omega 
              \; |\; t \in \pT^\mm_{n};  \omega \in b_{\lmu}  \}&\to B^{\lmu}_{\sspecht{}}\\
t \ox a^\mm_{n-l}\www\omega &\mapsto (t+ I^{<\mm}_{n})(b^\mm_{n}( a^\mm_{n-l}\www\omega \otimes ww^\star) )
\end{split}\end{equation}
 is a surjective and induces to a surjective
 $P^l_n$-module homomorphism from
 $G_\W \; \specht^{n-l}_{\lmu}$ to $\specht^n_{\lmu}$.
Hence
$dim( \specht^n_{\lmu} ) = dim(G_\W \; \specht^{n-l}_{\lmu})$.
}
\red{NB THIS is NOT Proven!!}

\mdef\label{lem:isoWS}\blu{Let
$\lmu \in \sqcup_{\mm\in \gammal\setminus\hl_n} \Lambda_\mm
             = \sqcup_{\mm\in\gamma^{l,n-l}} \Lambda_\mm$. Then \[X:=\{ \, ((t\otimes ww^\star)+ I^{<\mm}_n) \, \www\omega \; | \; t\in \pT^\mm_{n-l}, \; \omega \in b_{\lmu} \} \] is a bais of $\W P^l_n\W$-module $ \W\specht^n_{\lmu}$.\\
\proof  
For spanning  \beq\label{eq:WS}  \begin{split}
%\Specht  =
\W\specht^n_{\lmu} &= \W P^\mm_n a^\mm_n w^{ba}_{e_\mu}
    = \kk \{ \W t \www\omega \;|\; t \in T^\mm_n; \; \omega \in b_{\lmu}  \}\\
    &= \kk \{ \W( t +  I^{<\mm}_n)\www\omega \;|\; t \in \pT^\mm_n; \; \omega \in b_{\lmu}  \}\end{split}\eq 
By Lemma \ref{lem:1}-II for  $t \in \pT^\mm_n$ we have $\hashi(\W t)\leq \hashi(t)$.  If $\hashi(\W t)< \hashi(t)$ then Lemma \ref{lem:idbas1} implies $\W( t +  I^{<\mm}_n)= I^{<\mm}_n$. Otherwise, since $\W$ do not permute the propagating parts  of $t$ we have 
\[ \W( t +  I^{<\mm}_n)= \W t+ I^{<\mm}_n= \W t b^\mm_n a^\mm_n+ I^{<\mm}_n= p\otimes ww^\star + I^{<\mm}_n
\] }
For some $p\in \pT^\mm_{n-l}$, for example see the following fig
\begin{figure}[h]
\[
\includegraphics[width=6.04in]{latexdraw/WScongS.eps}
\]
\caption{Here $n=9, l=2,$ and $\mm=(1,2)$.    The  left most and the middle diagrams  are  examples of $\W(t+ I^{<\mm}_n)= I^{<\mm}_n$,   and the right most diagram  is an example of  $ \W(t+ I^{<\mm}_n) =p\otimes ww^\star + I^{<\mm}_n.$}
\end{figure}
\\\blu{Hence Equation \ref{eq:WS} becomes
\[= \kk \{ (( t\otimes ww^\star) +  I^{<\mm}_n)\www\omega \;|\; t \in \pT^\mm_{n-l}; \; \omega \in b_{\lmu}  \}\]
 The linear independence follows from  $X \subseteq  \{ \;  (p+I^{<\mm}_{n})\, \www\omega \; | \; p\in \pT^\mm_{n}, \; \omega \in b_{\lmu} \}.$  
 }
 
 
 
\mdef\label{lem:isoWSS}\blu{Let
$\lmu \in \sqcup_{\mm\in \gammal\setminus\hl_n} \Lambda_\mm
             = \sqcup_{\mm\in\gamma^{l,n-l}} \Lambda_\mm$. We have an isomorphism of $\W P^l_n\W$-modules:
$ \W\specht^n_{\lmu} \cong \specht^{n-l}_{\lmu}$.
\\\proof
Note from Lemma \ref{lem:isoWS} the set $X$ is  a basis of $ \W\specht^n_{\lmu}.$ The assignment
\begin{equation}\label{eqWBtoB} \begin{split}
  \theta: X &\to \{ \;  (p+I^{<\mm}_{n-l})\, \www\omega \; | \; p\in \pT^\mm_{n-l}, \; \omega \in b_{\lmu} \}\\
\left(\left( t\otimes ww^\star\right) +  I^{<\mm}_n\right)\www\omega &\mapsto (t+I^{<\mm}_{n-l})\, \www\omega
\end{split}\end{equation}
 is a set bijection since $|X|=|\pT^\mm_{n-l}\times  b_{\lmu}|=rank_K(\specht^{n-l}_{\underline{\mu}})$ (N.B. the $\www\omega$ on the right hand side of Equation \ref{eqWBtoB} is in the image of the map from $S_\mm$ to $P^l_{n-l}$  defined in Lemma~\ref{lem:groupc}). Further, the IBN property of $K$  implies that $\theta$ can be extended $K$-linearly to a $K$-module isomorphism between $ \W\specht^n_{\lmu} $ and $ \specht^{n-l}_{\lmu}$. It remains to show that the map $\theta$ also commutes with the action of $\W P^l_n\W$. 
 Let $p\otimes ww^\star\in \W P^l_n \W$ and $t\otimes ww^\star\in X $. Then 
 \begin{equation*}\begin{split} \theta((p\otimes ww^\star)( t\otimes ww^\star) +  I^{<\mm}_n)\www\omega))&=\theta(((pt\otimes ww^\star)+  I^{<\mm}_n)\www\omega)\\
 &=(pt + I^{<\mm}_{n-l})\www\omega=(p\otimes ww^\star)((t + I^{<\mm}_{n-l})\www\omega)\\
 &=(p\otimes ww^\star)\theta((t\otimes ww^\star + I^{<\mm}_{n})\www\omega)
 \end{split}
 \end{equation*}
 (N.B. in the first  equality a factor of $\delta$ is ignored and that is because when $\delta$ is not invertible in $K$ we can use $\W_b$ instead of $\W$)
 Hence $ \W\specht^n_{\lmu} \cong \specht^{n-l}_{\lmu}$ as $\W P^l_n\W$-modules.
}

%}}}
}}

%{{{ Proof

\mdef\blu{ Proof of \ref{lem:Gspecht}.
  Lemma \ref{lem:FWS} %\ref{lem:isoWSS}
implies that
$G_\W \; \specht^{n-l}_{\lmu} \cong P^l_n\W \ox \W \specht^n_{\lmu} $.
Note that there is  a surjective
$P^l_{n}$-module homomorphism form
$P^l_n\W \ox \W \specht^n_{\lmu}$
to $ P^l_n\W\specht^n_{\lmu}= \specht^n_{\lmu}$. By  Equation
\ref{eq:run4u} ??
$rank_K( \specht^n_{\lmu} ) \geq rank_K(G_\W \;  \specht^{n-l}_{\lmu})$.
Hence 
$
G_\W \; \specht^{n-l}_{\lmu}\cong \specht^n_{\lmu}.
$.
\qed
}


\medskip

%}}}

%{{{ Examples

\mdef
%\noindent
Examples.
Here are some examples in $G_W \specht^5_{((2,1),(1))} $
(for now using the $a$-version of  \blu{$W$ maybe $\W$}).
Note that by \ref{} we may formally `slide' any component carried on the first 5
tracks through the $\ox$ (although the factor represented actually
changes,
for example between a partition and a class of partitions, under such
a move).


For the first example consider Fig.\ref{fig:1x}.
We start with an element in the form 
$p (t\ot ww^*) \ox a \www{\be_1}$,
where $p \in P^2_7$ and
(abusing notation slightly) 
$\be_1 \in b_{(2,1)}$ is a basis
element of $\sspecht_{(2,1)}$ (and hence gives a basis element of 
$\sspecht_{((2,1),(1))}$).  
Let us number the lines 1-to-7 across the top. 
As an example of (a), note that the perm of 3 and
\blu{6} in $p$ can be considered as a perm in the last position
and can be ignored in $p(t \ot ww^*)$ due to the $ww^*$. 
As an example of (b),
the remaining crossings in $p$ can be slid to the first 5 tracks and
hence through the $\ox$ as shown in the middle expression.

As an example of (c) consider the following element $p \ox a^\mm e_1$.
Here the $p$ has propagating index $(3,0)$, compared to $\mm=(3,1)$.
In the middle expression $p$ is factorised with a factor of index
$(3,0)$ in the first 5 tracks
\[
\includegraphics[width=5.04in]{latexdraw/Gwz.eps}
\]
\[
\includegraphics[width=5.04in]{latexdraw/Gwzzz.eps}
\]

%}}}

%\red{END SANDPIT.}


%{{{ Local Variables

% Local Variables:
% folded-file: t
% End:

%}}}


==> tex/sandpit0.tex <==
% $Id: sandpit.tex,v 1.1 $

%{{{ ignored initial bit

\ignore{{
\noindent
\red{SANDPIT FILE! }

%\red{Nothing here yet! Write anything you like here.   :-) }

The following equations may help in proving the middle iso. 


$P^l_n \WW \ox P^l_{n-l} a^\mm_{n-l}= P^l_n \WW P^l_{n} \WW \ox a^\mm_{n-l}= P^l_n \WW 
 \ox a^\mm_{n-l}$


$P^l_n \WW ( P^{l}_{n-l} a^\mm_{n-l} \otimes 1_l )=P^l_n \WW a^\mm_{n}=P^l_n  a^\mm_{n}$
...
}}


%}}}

%{{{ CLAIM

\mdef CLAIM.
Consider choices for $d \in \mP^l_n$ at the first factor
in \eqref{eq:run4u}.
Then:
\\
(a) any non-trivial perm in the last positions (after $n-l$) can be ignored \\
(b) any earlier perm can be put to the right of the $\ox$  \\
(c) % any element
for $d \in I^{<\mm}_n$  %`goes to the right' as {\em zero}, i.e.
we have $d(t\otimes ww^\star)\ox a^\mm_{n-l}\www\omega=0$.
%\red{.... OK!?!?!}

%}}}
\newcommand{\ot}{\otimes}  %% name for diagram cat monoidal product
%{{{ fig

\newcommand{\be}{\beta}

\begin{figure}
\[
\includegraphics[width=5.04in]{latexdraw/Gw.eps}
\]
\caption{Example for claims (a,b) with $l=2$ and $n=7$.
Considering the leftmost picture of an element of form
$p (t\ot ww^\star) \ox a \www{\beta_1} $,
the middle box contains a
relative-noncrossing $t\ot ww^\star$.
The crossing of `lines' 3 and 6 in the top box % in the leftmost picture
is `in last positions'.
\label{fig:1x}}
\end{figure}

%}}}
%{{{ more

\redxx{AFter claim proof Need to come back and say what is the logic to
complete the proof of Lemma!
I think the logic is that overall we want to show that the left factor
ranges over $T^\mm_n$. --- Maybe it is clear that is ranges over at
least this much, and the arguments above show that it is no more?
}

%}}}

%\red{END SANDPIT.}


%{{{ Local Variables

% Local Variables:
% folded-file: t
% End:

%}}}


==> tex/sandpit1.tex <==
{{\mth 
%It follows from Lemma~\ref{lem:Gspecht}, Theorem~\ref{th:Ass1}, 
%and the construction that t
Suppose $k=\C$
and $\delta \neq 0$.
Recall the simple $P^l_n$-modules $L_{\lmu} = \head\specht^n_{\lmu}$
from (\ref{de:Llmu}). 
The modules
$\specht^n_{\lmu}$ have a  %%n upper
lower-unitriangular decomposition
matrix with respect
%to the partial order $(\Lambda(\Pl_n),>)$ \red{ ???}.
any order $\prec$ on  $\Lambda(P^l_n)$ in which
$\mm<\mm'$  implies
%%$\lmu \prec \lnu$
$\lnu \prec \lmu$
for
$\lmu \in \Lambda_\mm$ and $\lnu\in\Lambda_{\mm'}$.
}}
\proof
Recall that by  Theorem~\ref{th:index1} the pair $(\gammal , a^- )$ is a core of  $P^l_n$. When $k=\C$ for each $\lmu\in \Lambda_\mm$ the $\mmu$-Specht module $\sspecht_{\mmu}$  is simple as $\C S_\mm$-module.  By Equation~\ref{eq:spechtinflate} and Lemma~\ref{le:Diso} the set of modules $\{\specht^n_{\lmu}\mid \lmu \in \Lambda(P^l_n)\}$ are the corresponding $G$-functor $\Delta$-modules as in Equation~\ref{eq:Gdelta}. Now the result follows from  Lemma~\ref{Th:upperun}.\qed


==> tex/standard-chwas.tex <==

%% Chwas's expanded Lemmas for standard mod isomorphisms

\subsubsection*{Discussion 1}
%{{{ chwas 
 
%{\mlem\label{lem:S^p} If $p\in T^\mm$ then $S^p:=\{pw\;|\; w\in S_\mm\}$ is a basis of $pkS_\mm$. 
%}
%\proof The spanning  follows from the definition of  $pkS_\mm$. Note that $S^p\subseteq \mP^{\mm}_n$, hence by Lemma~\ref{lem:basis:mP^mm} the set   $S^p$ is linearly independent.
%\qed
{\mlem\label{lem:FM} Let $A$ be a finite dimensional $k$-algebra.  Let $M$ be a left ideal ${A}$-module  with a basis $B_M$ and $F$ be a right free $A$-module of finite rank with free basis $T$.  Then 
I) $FM=\bigoplus_{p\in T} p  M;$%\bigoplus_{p\in T^\mm} pa^\mm M;$ 
\\ II) for each $p\in T$ we have $dim( pM) =dim(M);$% $dim(P^\mm_n a^\mm M)=|T^\mm|\cdot|B_M|;$
 \\III)   the set $\{pw\;|\; p\in T ;w\in B_M\}$  is basis of $FM.$
 \\IV) $M' = F \otimes_{A} M$ has a basis with a factored form 
\[
B_M'  \; = \{ p \otimes w \; | \; p \in T ; \; w \in B_M  \}.
\]
}
\proof  
%\\Claim 1: For any $p\in T^\mm$ the set $S^p:=\{pw\;|\; w\in S_\mm\}$ is a basis for the vector space $pkS_\mm.$
I) First note that by the freeness of $F$ we have that $T A=FA$. Hence
 $$F M=TA M\subseteq +_{p\in T } p  M\subseteq F M,$$
 which implies that $FM =+_{p\in T} p M.$ To show the sum $+_{p\in T} p M$ is direct, 
%\\ 2) the sum is direct 
%\\1--- is true by a similar  argument  as in part I) of this Lemma.
let  $p, q\in T$ with $p\neq q$. Then $p  M\cap q  M\subseteq pA\cap qA$ since $M$ is a left ideal of $A$.  We have $pA\cap qA=  \{0\}$ since $p$ and $q$ are $A$-linearly independent.    Hence $p  M\cap q  M=\{0\}$  
%\\ Claim 3: for any $p\in T^\mm$ we have $dim( pa^\mm M) =dim(M)$.


II) 
\blu{another proof: To prove II it is enough to show that  $pB_M=\{pw\; |\; w\in B_M\}$ is a basis of $pM$, since $|B_M|=|pB_M|$. To this end, extend the basis  $B_M$ of $M$ to a basis of $A$, call it $B'_M$. Then $pB'_M=\{pw\; |\; w\in B'_M\}$ is a basis of $pA$, since it spans $pA$ and $dim(A)=dim(pA)$. Now $pB_M\subseteq pB_M'$ hence $pB_M$ is linearly independent. Hence  $pB_M$ is a basis of $pM$.}
  The set map
\begin{equation*}
\begin{split}
\mu_p:  B_M &\to p M\\
w&\mapsto pw
\end{split}
\end{equation*}
  can be extended  uniquely in to a linear map from $M$ to $p M$.  Further, the map $pw\mapsto w$ \blu{(do we
 need to say more about this map or it is okay like that?)}\blu{ the argument goes like this: First we show that that $pB_M$ is a basis of $pM$. To this end, extend the basis  $B_M$ of $M$ to a basis of $A$, call it $B'_M$. Then $pB'_M=\{pw\; |\; w\in B'_M\}$ is a basis of $pA$, since it spans $pA$ and $dim(A)=dim(pA)$. Now $pB_M\subseteq pB_M'$ hence $pB_M$ is linearly independent. Hence  $pB_M$ is a basis of $pM$. Then \begin{equation*}
\begin{split}
\mu'_p:  pB_M &\to  M\\
pw&\mapsto w
\end{split}
\end{equation*} is a set map  which 
   %Therefore, for each $pw_1,pw_2\in pB_M$ we have $pw_1=pw_2$ implies  $w_1=w_2.$
  }
  is the inverse of (the linear extension of ) $\mu_p$.  Hence $dim( p M) =dim(M)$. 


III) By part I the given set spans $ F  M.$ Again by using parts I and II of this Lemma   we have $dim(FM)=|T |\cdot|B_M |.$ Hence the set $\{pw\;|\; p\in T ;w\in B_M\}$ is linearly independent. 

IV) By the freeness of $F$ we have a spanning set of form $pw \otimes b$ with
$p \in T $, $w \in A$ and $b \in B_M$.
But $pw \otimes b = p \otimes wb$ so, fixing $p$, the set
$\{ p \otimes b \; : \;  b \in B_M \}$
spans the same space as
$\{ pw \otimes b \; : \; w\in A, b \in B_M \}$.
Thus the claimed set is spanning.
To see that it is independent note that $F$ is a free
right
$A$-module
%\red{(see (\ref{pa:freerightS}))}
with free basis $T$
%\red{can we not perhaps use this property in some more general way here?}
and so
(since $A \otimes_A {}_A M \cong M$) we have
$dim(M' ) = | T |\cdot|B_M |$.


\qed

%}}}
%{{{ chwas0 -commented

%{\mlem Let $M$ be a left ideal ${\kiss}$-module  with a basis $B_M.$ Then 
%\\I) $P^\mm a^\mm M=\bigoplus_{p\in T^\mm} p  M;$%\bigoplus_{p\in T^\mm} pa^\mm M;$ 
%\\ II) for each $p\in T^\mm$ we have $dim( pa^\mm M) =dim(M);$% $dim(P^\mm_n a^\mm M)=|T^\mm|\cdot|B_M|;$
% \\III)   the set $\{pw\;|\; p\in T^\mm;w\in B_M\}$  is basis of $ P^{\mm}_n a^{\mm}  M.$
%}
%\proof We identify $\kiss$ with $a^\mm P^{\mm}_n a^{\mm}$. 
%%\\Claim 1: For any $p\in T^\mm$ the set $S^p:=\{pw\;|\; w\in S_\mm\}$ is a basis for the vector space $pkS_\mm.$
%I) First note that by Lemma~\ref{lem:tranv1}  we have $T^\mm kS_\mm= P^\mm kS_\mm $. Hence
% $$P^\mm a^\mm M=T^\mm kS_\mm a^\mm M\subseteq +_{p\in T^\mm} pa^\mm M\subseteq P^\mm a^\mm M.$$
% Therefore,  $P^\mm a^\mm M =+_{p\in T^\mm} p M.$ To show the sum $+_{p\in T^\mm} p M$ is direct, 
%%\\ 2) the sum is direct 
%%\\1--- is true by a similar  argument  as in part I) of this Lemma.
%let  $p, q\in T^\mm$ with $p\neq q$. Then $pa^\mm M\subseteq pkS_\mm$ and $qa^\mm M\subseteq qkS_\mm$, since $M$ is a left ideal of $kS_\mm$. Note that $pa^\mm M\cap qa^\mm M\subseteq pkS_\mm\cap qkS_\mm$, hence to prove that the sum is direct it is enough to show that the last intersection is $\{0\}$.   By Lemma~\ref{lem:S^p} the spaces  $pa^\mm kS_\mm$ and $qa^\mm kS_\mm$  have basis $S^p$ and $S^q$.    Lemma~\ref{lem:polarPm} implies that $S^p\cap S^q=\emptyset.$ Hence $ pkS_\mm\cap qkS_\mm=\{0\}$.  
%%\\ Claim 3: for any $p\in T^\mm$ we have $dim( pa^\mm M) =dim(M)$.
%
%
%II)   The set map
%\begin{equation*}
%\begin{split}
%\mu_p:  B_m &\to pa^\mm M\\
%w&\mapsto pw
%\end{split}
%\end{equation*}
%  can be extended  uniquely in to a linear map from $M$ to $pa^\mm M$.  Further, the map $pw\mapsto p^\star p w=\delta^{c(p|p^\star)}a^\mm w=\delta^{c(p|p^\star)}w$ is the inverse of (the linear extension of ) $\mu_p$.  Hence $dim( pa^\mm M) =dim(M)$. 
%
%
%II) By part I the given set spans $ P^{\mm}_n a^{\mm}  M.$ Again by using parts I and II of this Lemma   we have $dim(P^\mm_n a^\mm M)=|T^\mm|\cdot|B_M|.$ Hence the set $\{pw\;|\; p\in T^\mm;w\in B_M\}$ is linearly independent. 
%\qed

%}}}
%{{{ chwas

{\mlem{ \label{de:basMM} \label{lem:basisc} \label{lem:ny1}
%From Lem.\ref{lem:tranv1} we have the following.
Let  $A,M$ and $F$ be as given in Lemma~\ref{lem:FM}.   
%where $M$ is a  %left ideal
%\red{the proof does not use ideal property. omit? (it uses freeness)}
%${\kiss}$-module,
%where $B_M$ is a basis for $M$.
Let $B$ be finite dimensional algebra.  If $F$ is  an $A$-$B$-bimodule and $M$ is a left ideal $A$-module then
  the surjective multiplication map
$\mu: p \otimes w \mapsto pw \in FM$
   is injective, so $$ F \otimes_{A} M\cong  F  M$$  as left $B$-modules. %\blu{I think this problem is resolved and we should remove the red tag}
}}
\proof%We identify $\kiss$ with $a^\mm P^{\mm}_n a^{\mm}$. 
If $M$ is a left ideal $A$-module then   the set map 
\begin{equation*}
\begin{split}
F \times M&\to FM\\
(p,w)&\mapsto pw
\end{split}
\end{equation*}
is $A$-balanced. Hence by the universal property of tensor products there exists a group homomorphism
\begin{equation*}
\begin{split}
\mu:F \otimes M&\to F M\\
p\otimes w&\mapsto pw.
\end{split}
\end{equation*}
%
%
%  $\mu: p \otimes w \mapsto pw \in P^{\mm}_n a^{\mm} M$. 
  Further, for any $q\in B$ we have 
$$\mu(q(p\otimes w))=\mu(qp\otimes w))=(qp)w=q(pw)=q\mu(p\otimes w)$$
  hence  $\mu$ is a left $B$-module morphism.
%  Finally,
By Lemma~\ref{lem:FM}
$FM$ and $ F \otimes_{A} M  $ have the same dimension, hence surjectivity of $\mu$ implies that $\mu$ is injective.
%}}}
\red{NB A lot of commented out stuff here.}
%{{{ commented out part (chwas/paul)
%  \red{proof?
%    first we claim the given set is spanning
%    (why? probably argument similar to above works).
%    second
%    ... consider 
%A SOMEHOW LINEARIZED 
%    ket-c-bra (cf. bra-c-ket)
%    decomposition of this set as in \eqref{eq:ketcbra}.
%    By assumption the elements have the form
%    $p\Sigma_i c_i w_i = \Sigma_i c_i p  w_i$ where each $w_i \in
%    S_\mm$ and $c_i \in k$.  ...
%    we claim that this takes $pw \mapsto (p,w,1)$.
%    Thus the map $(p,w) \mapsto pw$ is invertible and the two bases
%    have the same order.
%  }
%
%the following is the older version of the above theorem
%I). By Lemma~\ref{lem:tranv1}  we have a spanning set of form $pw \otimes b$ with
%$p \in T^\mm$, $w \in S_\mm$ and $b \in B_M$.
%But $pw \otimes b = p \otimes wb$ so, fixing $p$, the set
%$\{ p \otimes b \; : \;  b \in B_M \}$
%spans the same space as
%$\{ pw \otimes b \; : \; w\in S_\mm, b \in B_M \}$.
%Thus the claimed set is spanning.
%To see that it is independent note that $P^\mm_n a^\mm$ is a free
%right
%$k S_\mm$-module
%\red{(see (\ref{pa:freerightS}))}
%with free basis $T^\mm$
%\red{can we not perhaps use this property in some more general way here?}
%and so
%(since $A \otimes_A {}_A M \cong M$) we have
%$dim(M' ) = | T^\mm |.|B_M |$.
%
%II). We identify $\kiss$ with $a^\mm P^{\mm}_n a^{\mm}$. If $M$ is a left ideal ${\kiss}$-module then $P^{\mm}_n a^{\mm} M$ is defined and the set map 
%\begin{equation*}
%\begin{split}
%P^{\mm}_n a^{\mm} \times M&\to P^{\mm}_n a^{\mm} M\\
%(p,w)&\mapsto pw
%\end{split}
%\end{equation*}
%is ${\kiss}$-balanced. Hence by the universal property of tensor products there exists a group morphism
%\begin{equation*}
%\begin{split}
%\mu:P^{\mm}_n a^{\mm} \otimes M&\to P^{\mm}_n a^{\mm} M\\
%p\otimes w&\mapsto pw.
%\end{split}
%\end{equation*}
%%
%%
%%  $\mu: p \otimes w \mapsto pw \in P^{\mm}_n a^{\mm} M$. 
%  Further, for any $q\in P^\mm_n$ we have 
%$$\mu(q(p\otimes w))=\mu(qp\otimes w))=(qp)w=q(pw)=q\mu(p\otimes w)$$
%  hence  $\mu$ is a left $P^{\mm}_n$-module morphism.
%%  Finally,
%  Next,
%\red{we claim that} 
%  the set $\{pw\;|\; p\in T^\mm;w\in B_M\}$ is a basis of
%  $P^{\mm}_n a^{\mm} M$,
%  \red{proof?
%    first we claim the given set is spanning
%    (why? probably argument similar to above works).
%    second
%    ... consider 
%A SOMEHOW LINEARIZED 
%    ket-c-bra (cf. bra-c-ket)
%    decomposition of this set as in \eqref{eq:ketcbra}.
%    By assumption the elements have the form
%    $p\Sigma_i c_i w_i = \Sigma_i c_i p  w_i$ where each $w_i \in
%    S_\mm$ and $c_i \in k$.  ...
%    we claim that this takes $pw \mapsto (p,w,1)$.
%    Thus the map $(p,w) \mapsto pw$ is invertible and the two bases
%    have the same order.
%  }
%  \blu{Second, let 
%  $$\sum_{p\in T^\mm, w\in B_M} \alpha_{p,w}pw=0,$$ 
%  with $\alpha_{p,w}\in k$ for each $p\in T^\mm$ and $w\in B_M$. Then 
%  $$0=\sum   \alpha_{p,w}pw=\sum   \alpha_{p,w}p(\sum_i c_{i,p,w}w_i)=\sum \sum\alpha_{p,w} c_{i,p,w}pw_i,$$
%   where $w_i$ run over the elements of  $S_\mm$ and $c_{i,p,w}\in k$. [I am not sure bout this step ]Since each $pw_i\in B^\mm$ (note Lemma~\ref{lem:tranv1}) we have  $\alpha_{p,w} c_{i,p,w}=0$. Now if there is $p\in T^\mm$ and $w\in B_M$ such that $\alpha_{p,w}\neq 0$ then we get $c_{i,w,p}=0$ for all $i$. Hence there is  $w\in B_M$ such that $w=\sum c_{i,p,w}w_i=0$, which is a contradiction. Thus the set  $\{pw\;|\; p\in T^\mm;w\in B_M\}$  is linearly independent.}
%  \red{explain! use surjectivity?}
%  shows that $\mu$ is injective. 
%If $M$ is ideal then the multiplication map $b \otimes w \mapsto bw$
%is an isomorphism.
%\red{!finish me! independence??}
%The idea is that the group part of the original basis $B^\mm$ is absorbed
%and replaced by the module.
%}}}
%{{{ more
\qed

{\mlem{ \label{de:basM1} \label{lem:basisc} \label{lem:ny1}\blu{Corollary?}
%From Lem.\ref{lem:tranv1} we have the following.
(I) Any $P^\mm_n$-module of form 
\[
M' = P^{\mm}_n a^{\mm} \otimes_{\kiss} M
\]
where $M$ is a  %left ideal
%\red{the proof does not use ideal property. omit? (it uses freeness)}
${\kiss}$-module,
has a basis with a factored form 
\[
B_M^{\mm} \; = \{ p \otimes w \; | \; p \in T^{\mm}; \; w \in B_M \}
\]
where $B_M$ is a basis for $M$.

(II) If $M$ is a left ideal ${\kiss}$-module then
%\red{ the surjective multiplication map
%$\mu: p \otimes w \mapsto pw \in P^{\mm}_n a^{\mm}  M$
%   is injective, so 
$M' \cong  P^{\mm}_n a^{\mm}  M$ as left $P^{\mm}_n$-modules.
% \blu{I think this problem is resolved and we should remove the red tag}
}}

\proof Part I is a special case of part IV of Lemma~\ref{lem:FM}.  II) By  Lemma~\ref{lem:tranv1} the right $\kiss$-module $P^\mm a^\mm$ is free, now use Part II of Lemma~\ref{de:basMM}. 
\qed
%Is this OK, or do we need $M$ to be a left ideal (which is
%enough for us)? ...

%}}}
\subsubsection*{End discussion 1}


%{{{ Local Variables
% Local Variables:
% folded-file: t
% End:
%}}}


==> tex/uni-chwas.tex <==
\ignore{{Let $\preceq$ be  a linear  order relation on $\Lambda(A)$ such that $|\mu|<|\nu|$ in $(\gamma,\leq)$ implies  $\mu\prec \nu$.   \ignore{{ that is $(\Lambda(A), \preceq)$ is totally ordered set.
The relation $\leq$ on $\gamma$ induces a partial order relation, say  $\preceq$,  on  $\Lambda(A)$  in the following way; for $\mu, \nu \in \Lambda(A)$ we have $\mu\prec \nu$ if and only if $|\mu|<|\nu|$ in $(\gamma,\leq).$ }}
Let $d^\gamma_{_{\mu x}}:=[\Delta_\mu : L_x ]$. 
 Let the rows of the matrix 
$(d^\gamma_{\mu x})=:D_{A}^\gamma$ be labelled by the elements of $\Lambda(A)$ increasingly according to $\preceq$. Then $D^\gamma_A$ has only 1's on the main diagonal and it is block upper unitraingular, but it is not necessarily unitriangular.
\proof Let $\mu\in \Lambda(A)$. Then   $d^\gamma_{_{\mu \mu}}\neq0$ by part I. Further, part II implies $d^\gamma_{_{\mu \mu}}=1.$ If $d^\gamma_{_{\mu x}}\neq0$ and $\mu\neq x$ then by part II we have $e_{|\mu|} L_x = 0$. Hence either $\mu   \prec x$ or they are not related with respect to $\preceq.$
\mdef  If one let $e_\lambda=1$ for all $\lambda\in\gamma$ (cf. with the remark after Theorem~\ref{th:genLam}) then Lemma~\ref{uni:lem} is trivial and $D^\gamma_A$ is going to become the identity matrix. }}
%
%
\label{Th:upperun}Let $A$ be a $k$-algebra and $(\gamma, e_-)$ be a core for $A$.   Let $D_{A}^\gamma:=(d^\gamma_{\mu x})$ with $d^\gamma_{\mu x}=[\Deltag_\mu : L_x ].$
\ignore{\red{If $e_\lambda A^\lambda e_\lambda$ is semisimple for each $\lambda\in\gamma$ then}} 
The matrix $D_{A}^\gamma$ is upper-unitriangular with respect to any order $<'$ on $\Lambda(A)$ in which $ \ccc{\mu}<\ccc{x}$   in $\gamma$  implies $\mu <' x$.
\proof Let $\mu\in \Lambda(A)$. First note that  $d^\gamma_{_{\mu \mu}}\neq0$ by part 
I of Lemma~\ref{lem:unitri0} . Further, part II of \ref{lem:unitri0} implies 
$d^\gamma_{_{\mu \mu}}=1.$ Let $x\in \Lambda(A)$ with $x\neq \mu$. If 
$d^\gamma_{_{\mu x}}\neq0$ then $e_{\ccc{x}}\Deltag_\mu\not=0$. Hence by the axiom 
(AI) of the definition of core we have $\ccc{\mu}\leq \ccc{x}.$ Note that again  by part II 
of Lemma~\ref{lem:unitri0} we have $e_{\ccc{\mu}} L_x = 0$. Hence we cannot have 
$\ccc{x}=\ccc{\mu}$ otherwise we would get $e_{\ccc{\mu}} L_x \not= 0$. Therefore  $ 
\ccc{\mu}< \ccc{x}.$ 

\ignore{Hence either $\mu   <' x$ or they are not related with respect to $<'.$ If  $\mu$ and $x$ are not related   then $|\mu|\neq|x|$  otherwise we would get $e_{|\mu|} L_x \not= 0$.
Now what if $|\mu|$ and $|x|$ are not related. Then by axiom (AI) of the definition of core we get $e_{|x|}\Delta_\mu=0$ }
\ignore{\red{if we assume $\gamma$ is a chain then either $|\mu|=|x|$(which is not possible by the above paragraph) or $|\mu|<|x|$. Hence $\mu<'x.$ }}






==> tex/uni-was.tex <==
\ignore{{Let $\preceq$ be  a linear  order relation on $\Lambda(A)$ such that $|\mu|<|\nu|$ in $(\gamma,\leq)$ implies  $\mu\prec \nu$.   \ignore{{ that is $(\Lambda(A), \preceq)$ is totally ordered set.
The relation $\leq$ on $\gamma$ induces a partial order relation, say  $\preceq$,  on  $\Lambda(A)$  in the following way; for $\mu, \nu \in \Lambda(A)$ we have $\mu\prec \nu$ if and only if $|\mu|<|\nu|$ in $(\gamma,\leq).$ }}
Let $d^\gamma_{_{\mu x}}:=[\Delta_\mu : L_x ]$. 
 Let the rows of the matrix 
$(d^\gamma_{\mu x})=:D_{A}^\gamma$ be labelled by the elements of $\Lambda(A)$ increasingly according to $\preceq$. Then $D^\gamma_A$ has only 1's on the main diagonal and it is block upper unitraingular, but it is not necessarily unitriangular.
\proof Let $\mu\in \Lambda(A)$. Then   $d^\gamma_{_{\mu \mu}}\neq0$ by part I. Further, part II implies $d^\gamma_{_{\mu \mu}}=1.$ If $d^\gamma_{_{\mu x}}\neq0$ and $\mu\neq x$ then by part II we have $e_{|\mu|} L_x = 0$. Hence either $\mu   \prec x$ or they are not related with respect to $\preceq.$
\mdef  If one let $e_\lambda=1$ for all $\lambda\in\gamma$ (cf. with the remark after Theorem~\ref{th:genLam}) then Lemma~\ref{uni:lem} is trivial and $D^\gamma_A$ is going to become the identity matrix. }}
%
%
\label{Th:upperun}Let $A$ be a $k$-algebra and $(\gamma, e_-)$ be a core for $A$.   Let $D_{A}^\gamma:=(d^\gamma_{\mu x})$ with $d^\gamma_{\mu x}=[\Deltag_\mu : L_x ].$
\ignore{\red{If $e_\lambda A^\lambda e_\lambda$ is semisimple for each $\lambda\in\gamma$ then}} 
The matrix $D_{A}^\gamma$ is upper-unitriangular with respect to any order $<'$ on $\Lambda(A)$ in which $ \ccc{\mu}<\ccc{x}$   in $\gamma$  implies $\mu <' x$.
\proof Let $\mu\in \Lambda(A)$. First note that  $d^\gamma_{_{\mu \mu}}\neq0$ by part 
I of Lemma~\ref{lem:unitri0} . Further, part II of \ref{lem:unitri0} implies 
$d^\gamma_{_{\mu \mu}}=1.$ Let $x\in \Lambda(A)$ with $x\neq \mu$. If 
$d^\gamma_{_{\mu x}}\neq0$ then $e_{\ccc{x}}\Deltag_\mu\not=0$. Hence by the axiom 
(AI) of the definition of core we have $\ccc{\mu}\leq \ccc{x}.$ Note that again  by part II 
of Lemma~\ref{lem:unitri0} we have $e_{\ccc{\mu}} L_x = 0$. Hence we cannot have 
$\ccc{x}=\ccc{\mu}$ otherwise we would get $e_{\ccc{\mu}} L_x \not= 0$. Therefore  $ 
\ccc{\mu}< \ccc{x}.$ 

\ignore{Hence either $\mu   <' x$ or they are not related with respect to $<'.$ If  $\mu$ and $x$ are not related   then $|\mu|\neq|x|$  otherwise we would get $e_{|\mu|} L_x \not= 0$.
Now what if $|\mu|$ and $|x|$ are not related. Then by axiom (AI) of the definition of core we get $e_{|x|}\Delta_\mu=0$ }
\ignore{\red{if we assume $\gamma$ is a chain then either $|\mu|=|x|$(which is not possible by the above paragraph) or $|\mu|<|x|$. Hence $\mu<'x.$ }}





